Adversarial Search and Tracking with Multiagent Reinforcement Learning in Sparsely Observable Environment

We study a search and tracking (S&T) problem where a team of dynamic search agents must collaborate to track an adversarial, evasive agent. The heterogeneous search team may only have access to a limited number of past adversary trajectories within a large search space. This problem is challenging for both model-based searching and reinforcement learning (RL) methods since the adversary exhibits reactionary and deceptive evasive behaviors in a large space leading to sparse detections for the search agents. To address this challenge, we propose a novel Multi-Agent RL (MARL) framework that leverages the estimated adversary location from our learnable filtering model. We show that our MARL architecture can outperform all baselines and achieves a 46% increase in detection rate.

==> arxiv_submission/background.tex <==
\subsection{Related Work \label{sec:BG}}
%Many related works are about the topic and could be cross-classified
%using the criteria of if using the visual memory or SLAM, the controller
%type and uncertainty analysis methods.

%General description. Here we need to describe how the following related
%works are organized. The papers we discussed here could be roughly
%cross-categorized using the criteria if the visual memory is neccessary,
%the controller type and if using globally optimization techniques like
%SLAM or using other visual servoing uncertainty analysis methods.
%Therefore, the related papers could be classified as: 1. Teach and
%repeat 2. Traditional visual servoing 2.1 IBVS 2.2 PBVS 2.3 Other
%advanced VS 3. Visual SLAM with Navigation 4. Visual servo uncertainty
%etc. These are parallel aspects from which we could analyze each paper,
%so maybe one paper will appear in more than one times in the following
%bullets.%

\subsubsection{Visual Teach and Repeat\label{sec:BG_vtr}}
%Evidence that visual features can support trajectory tracking or
%consistent navigation through space lies in the {\em Visual Teach and
%Repeat} (VTR) navigation problem in robotics 
%\cite{SEGVIC2009172,inproceedingsNwL}. 
%Given data or recordings of prior passes through an environment robots
%can reliably retrace past trajectories. It is achieved by creating a
%a visual map or a sense for the optical flow, along the trajectory, which
%is encoded into a VTR data structure and control algorithm\cite{6816849,KIDONO2002121}.
%Extensions include real-time construction of the VTR data structure
%during the teaching process, and the maintenance and updating of the VTR
%data during repeat runs \cite{High,8967994}.  Visual data in the form of
%feature points can have task irrelevant and relevant features, which
%provides VTR algorithms an opportunity to select the subset that best
%contributes to the localization or path following tasks \cite{8967994,longrange}. In the repeating phase, the descriptor of the features could also be improved to make the feature matching more robust to the environment change\cite{KRAJNIK2017127,10.1007/s10846-015-0320-1}. In summary, maintaining a consistent long term visual map and robust feature matching are core requirements for VTR. These constraints prevent this method from applying to real-time planning and navigation since it doesn't allow the system to obtain the prior visual knowledge under human control.
%Instead of recording videos along a certain trajectory in teaching phase,
%\cite{High} constructs a visual map of a certain area represented as a
%graph of linked images. 
%To adapt to the environment change, obsolete features are removed and new
%features are added into feature maps in \cite{8967994}. 
%It also selects the feature points with the best conditioning to
%localize. \\




Evidence that visual features can support trajectory tracking or
consistent navigation through space lies in the {\em Visual Teach and
Repeat} (VTR) navigation problem in robotics 
\cite{SEGVIC2009172,inproceedingsNwL}. 
Given data or recordings of prior paths through an environment, robots
can reliably retrace past trajectories.
The teaching phase of VTR creates a visual map that contains features
associated with robot poses obtained from visual odometry 
\cite{SEGVIC2009172,8967994,High,longrange,KRAJNIK2017127}. 
Extensions include real-time construction of the VTR data structure during the teaching process, and the maintenance and updating of the VTR data during repeat runs \cite{High,8967994}.  
Feature descriptor improvements make the feature matching more robust to
the environment changes \cite{KRAJNIK2017127,8460674}.
Visual data in the form of feature points can have task relevant and irrelevant features, which provide VTR algorithms an opportunity to select a subset that best contributes to the localization or path following task \cite{8967994,longrange}. 
While visual map construction seems similar to visual SLAM, map
construction is usually not dynamic; it is difficult to construct or
update visual map in real-time while in motion because of the
separation of the teach and repeat phases.  In addition, VTR focuses
more on local map consistency and does not work toward global pose
estimation \cite{longrange} since the navigation problems it solves are
usually defined in the local frame.

Another type of VTR uses the optical flow
\cite{inproceedingsNwL,10.1007/s10846-015-0320-1} or feature
sequence \cite{KIDONO2002121,6816849,5649557} along the trajectory,
which is then encoded into a VTR data structure and control algorithm
in the teaching phase.  Although this method is similar to visual
servoing, the system is largely over-determined.  It can tolerate 
feature tracking failure, compared with traditional visual
servo system, but may lead to discontinuities \cite{1389589}.  
Though this method handles long trajectories, and may be be supplemented
from new teach recordings, it can only track taught trajectories.


%\toedit{BAD TEXT:
%In summary, even though teach and repeat could guarantee a
%relative long-term navigation, it could not do online planning.
%Simutaneously, the tracking result will not be accurate since this method
%is not robust to suddenly environment changing and it is difficult to
%decide which image to track due to the inaccuracy of localization or the
%image appearance. NEED BETTER TRANSITION.}


%Comment on Teach and Repeat: Teach and repeat method needs the memory or
%the prior knowledge of the environment. The features used to navigate
%the robot are extracted using the pre-recorded videos or pre-constructed
%feature maps. Even though such method could guaranteen a relative
%long-term navigation, it could only plan offline and not robust to
%environment changing.

%Some existing navigation approaches with visual data are in the
%teach-and-repeat mode. Describe the similiarity and difference with each
%other and how they inspire our work.

\subsubsection{Visual Servoing\label{sec:BG_vs}}

Visual servoing (VS) has a rich history and a diverse set of strategies for
stabilizing a camera to a target pose described visually. VS algorithms
are classified into one of two categories:
image based visual servoing (IBVS) and 
position based visual servoing (PBVS)\cite{4015997,4141039}. 
IBVS implementations include both feature stabilization and feature
trajectory tracking \cite{4141039,1044366}.
%This idea could be dated back to \cite{1044366}, where the key idea is to
%use the local stability and robustness of image-based servoing by
%specifying adequate trajectories to follow in the image. 
As a feedback strategy IBVS regulation does not guarantee what path is
taken by the robot since the feature space trajectory has a nonlinear
relationship with the Cartesian space trajectory of the robot.
%However, there is no guaranteen that what the spatial trajectory will
%look like since the feature trajectory is not generated using trajectory
%in Cartesian space. 
Identifying a feature path to track based on a target Cartesian space
trajectory requires mapping the robot frame and the target positions into
the image frame over time to generate the feature trajectory
\cite{1044366,6564708}, precisely what is done here.
%To solve this problem, we need to predict what the camera will see along
%the planned spatial trajectory and generate feature trajectory based on
%this \cite{6564708}.

The target application is trajectory tracking for a mobile robot.
Mobile robots have been studied as candidates for visual servoing
\cite{SEGVIC2009172,inproceedingsNwL,cherubini:hal-00639659,9197114,1642112,5740604,1570628}.
Some of them use IBVS but do not use the full IBVS equations involving
the image Jacobian.  The centroid of the
features \cite{SEGVIC2009172}\cite{5740604}, the most frequent horizontal
displacement of the matched feature pairs \cite{inproceedingsNwL} or other
qualitative cost functions \cite{1642112} are used to
generate \cite{SEGVIC2009172} or correct \cite{inproceedingsNwL} the
feedforward angular velocity of mobile robot. 
These simplifications are reasonable since the lateral displacement of
the features reflects task relevant movement to be regulated by the
robot.  However, they are best suited to circumstances with higher
inaccuracy tolerance such as an outdoor, open field navigation.  We use
more precise velocity relations between the robot and feature motion to
generate a feedback control signal for exact tracking similar to
\cite{cherubini:hal-00639659}. %which was experimentally verified.
%shows an acceptable error in real experiment. 
That work studied the path reaching problem with a visible path, which
does not hold here. 

%Briefly introduce the traditional visual servoing. Here we could describe the concept of IBVS, PBVS and other VS methods and cite some theoritical paper (like Prof.Hutchison's visual servoing series) to help illustration.

%Show the applications for nonholonomic robot. Here we could cite some more practical papers which concentrate more on the real robot experiment.

%Comment on how our work is related to visual servoing.

\subsubsection{Navigation Using Visual SLAM\label{sec:BG_slam}}
%Similiar to the previous works in our lab, we also investigate the least-square problem to find how each feature could contribute to the final solution\cite{8593641}\cite{10.1007/978-3-030-01216-8_32} and  benchmark our proposed trajectory tracking method using turtlebot with a stereo camera in the ROS kinetic+Gazebo environment to show the performance against other controllers we created before statistically\cite{zhao2020closedloop}. A real robot experiment is also added to test the validity of our method. 

%This part shows the existed navigation strategies through visual SLAM. Remains to be seen what papers could be put here...
\begin{comment}
Simultaneous localization and mapping (SLAM) systems estimate the
robot's trajectory and world structure as the robot moves through space
\cite{4160954,4538852,10.1007/s11263-011-0466-7,7780809,6126513,%
10.1007/978-3-642-15986-2_2,10.1007/978-3-319-10605-2_54,photom,7898369,%
7219438,7946260,campos2020orbslam3}.
For some autonomous robots, the SLAM pose estimates provide good
signals for using pose-based feedback to track trajectories using
standard control policies. Generically though, the problem associated
to reliance on SLAM is the potential to accrue large estimation drift,
which will undermine precise trajectory tracking and goal attainment.

ORB-SLAM 1-3 \cite{7219438,7946260,campos2020orbslam3}. 
The reason why navigation systems need the help of SLAM is that it will
inevitably require its local or global pose as the feedback
information. 

There are many works intended to investigate the pose estimation
accuracy of each SLAM
system\cite{8460558,8964284,7140009,8436423,8794369,8460664,%
10.1007/978-3-030-33950-0_12,05c869ea074b4bc3b4a4ccf4c2692f83}. 
Most of them are tested only on the open-loop conditions, i.e. they only analyze the pose estimation difference with the ground truth trajectory and never care about the error when using the estimated pose to control. These benchmarking results are performed on different datasets \cite{8460558,8964284}, different computational resources \cite{7140009,8436423,8460664} and different maps\cite{10.1007/978-3-030-33950-0_12,05c869ea074b4bc3b4a4ccf4c2692f83}with different visual SLAM methods. These works build a norm for pose estimation error analysis and show the results in multiple configurations.  
\color{black}
\end{comment}

Visual simultaneous localization and mapping (V-SLAM) systems estimate
the robot's trajectory and world structure as the robot moves
through space \cite{cadena2016past}.  
For some autonomous robots, the SLAM pose estimates provide good
signals for using pose-based feedback to track trajectories using
standard control policies. The problem associated to reliance on SLAM
is the potential to accrue large estimation drift, which degrades
trajectory tracking and goal attainment.

%the SLAM pose estimates provide good pose-based feedback signal 
%to trajectory tracking using standard control policies. 
%One problem of being reliant on V-SLAM is that SLAM systems 
%may have large estimation drift, which will undermine the precision of 
%trajectory tracking. 
Pose estimation accuracy of SLAM is a major area of study
\cite{8964284,7140009,8436423,8794369,8460664}. 
% drop some redundant citations here? e.g. only need SLAMBench3 (no SLAMBench1/2); remove 39 & 40 since these are dataset paper.
However, most studies only test under open-loop conditions \cite{8964284,7140009,8436423,8460664}, 
i.e., they only analyze the pose estimation difference with the ground
truth trajectory, and do not consider the error induced when the
estimated pose informs feedback control. 
More recently, closed-loop evaluation of V-SLAM algorithms as part of
the feedback control and navigation system are tested for individual
SLAM systems \cite{cvivsic2018soft,WeEtAl_VIOSwarm[2018],lin2018autonomous} 
or across different systems \cite{zhao2020closednav}. Closed-loop
studies expose the sensitivity of pose-based feedback control and
navigation, e.g., sensitivity to V-SLAM estimation drift and latency.  
Our work builds upon an existing closed-loop benchmarking framework 
and shows sensitivity reduction over conventional pose-based
closed-loop navigation solution.  The proposed \textit{trajectory
servoing (TS)} method is not tied to a specific V-SLAM implementation.
%the sensitivity reduction is general and applicable to other navigation
%systems.
%However, only limited number of works are about the benchmarking with a closed loop visual SLAM system, i.e. using the estimated pose as the feedback in the trajectory tracking and test the error between the robot trajectory and desired one \cite{softslam,8276634}. The closed loop performance of visual SLAM is extremely important in the navigation since it reflects the accuracy of real trajectory tracking problems. Therefore, our lab makes much effort on this branch. \cite{Ye_Zhao_Vela_2019} proposes to use a decision tree to identify challenging benchmark properties from the characterization of selected sequence properties (scene, duration, motion dynamics  environment dynamic, revisit freqency). Based on multiple characterizations, \cite{9197003} designs a feedback controller using the estimated pose fused from MultiSensor-Fusion Extended Kalman Filter (MSF-EKF)\cite{9197003,20.500.11850/52698}. Even though this paper shows the possible reasons why the drift error will happen, it doesn't give the solution to overcome the drift error. This is the main topic of our paper.

%\subsection{Visual Navigation Using Non-Point Features}
%Papers using features other than points or other coordinate systems



==> arxiv_submission/conc.tex <==
\section{Conclusion \label{sec:con}}

%Closing statement. It should 1. objectively judge the advantages and disadvantages of our work and other's work. 2. Emphasis our contributions to use IBVS for non-holonomic robot navigation. 3. Talk about future work about using this method to achieve more functions like avoiding obstacle, help SLAM localization and etc..

In the paper, we presented a vision-based navigation approach for a
non-holonomic mobile ground robot called {\em trajectory servoing},
which combines the IBVS and V-SLAM.  This trajectory tracking method can
successfully follow a given short trajectory without externally derived
robot pose information. 
By integrating with estimated robot poses from V-SLAM, it can achieve
long-term navigation.  The V-SLAM system also provides robust feature
tracking to support stable trajectory servoing.
Experiments demonstrated improved tracking accuracy over pose-based trajectory 
tracking using estimated SLAM poses.

Future work intends to implement trajectory servoing approach on a real
Turtlebot platform to evaluate its performance. We also plan to perform
uncertainty analysis on the trajectory servoing feedback equations to
provide robustness to real-world measurement errors, which will also
aid in matching simulation performance outcomes to actual performance. 
%Moreover, the ground truth pose of robot is hard to obtain
%in reality. This may be solved by a Vicon motion capture system or other
%pose estimation methods. After working out these topics, we believe
%trajectory servoing will have a good tracking performance without
%explicit localization.


==> arxiv_submission/figs/trajservo_demo.tex <==
\tikzstyle{newline} = [-, thick]
\tikzstyle{newline_dashed} = [-, thick, dashed]
\tikzstyle{newtip} = [->, thick]
\tikzstyle{newtip_dashed} = [->, thick, dashed]
\tikzstyle{block} = [draw, rectangle, dashed, thick,rounded corners=2pt,
                     minimum height=1.5em, minimum width=5em, inner sep=4pt]

\newcommand{\figPose}[1]
{
\begin{tikzpicture}
  \node (r1) at (0,0) {};
  \node (r2) at (3,-1) {};
  \node (r3) at (0,-2) {};
  
  \draw[very thick] (r1.center) -- (r2.center) -- (r3.center) -- cycle;
  
  \fill[fill=#1] (r1.center)--(r2.center)--(r3.center);
\end{tikzpicture}
}

\tikzstyle{features}=[star, draw, inner sep=1pt]
  
  
\begin{tikzpicture}[inner sep=0pt, outer sep=0pt, auto, >=latex]
  % reference traj
  \node[anchor=west, scale=0.3] (refp1) at (0,0) {\figPose{red!60}};
  \node[anchor=west, scale=0.3] (refp2) at ($(refp1.east) + (0.7in, 0in)$) {\figPose{red!60}};
  \node[anchor=west, scale=0.3] (refp3) at ($(refp2.east) + (0.7in, 0in)$) {\figPose{red!60}};
  
  % real traj
  \node[anchor=north, scale=0.3] (realp1) at ($(refp1.south) + (0in, -1in)$) {\figPose{gray!40}};
  \node[anchor=north, scale=0.3] (realp2) at (realp1.north-|refp2.south) {\figPose{gray!40}};
  \node[anchor=north, scale=0.3] (realp3) at (realp1.north-|refp3.south) {\figPose{gray!40}};
  
  % ref features
  \node[features, fill=red!60, anchor=north, scale=2] (reff1) at ($(refp1.south) + (0in, -0.4in)$) {};
  \node[features, fill=red!20, anchor=north, scale=2] (reff2) at (reff1.north-|refp2.south) {};
  \node[features, fill=red!20, anchor=north, scale=2] (reff3) at (reff1.north-|refp3.south) {};
  
  % cur features
  \node[features, fill=gray!40, anchor=south, scale=2] (curf1) at ($(realp1.north) + (0in, 0.3in)$) {};
  \node[features, fill=gray!40, anchor=south, scale=2] (curf2) at (curf1.south-|realp2.north) {};
  \node[features, fill=gray!40, anchor=south, scale=2] (curf3) at (curf1.south-|realp3.north) {};
  
  % ref arrows
  \draw[newtip] ($(refp1.east) + (0.05in,0in)$) -- ($(refp2.west) + (-0.1in,0in)$);
  \draw[newtip] ($(refp2.east) + (0.05in,0in)$) -- ($(refp3.west) + (-0.1in,0in)$);
  
  % ref features
  \draw[newline] ($(refp1.south) + (0in,0in)$) -- ($(reff1.north) + (0in,0.1in)$);
  \draw[newtip_dashed] ($(reff1.north) + (0in,0.1in)$) -- ($(refp2.south) + (0in,0in)$) {};
  \draw[newtip_dashed] ($(reff1.north) + (0in,0.1in)$) -- ($(refp3.south) + (0in,0in)$) {};
  
  \draw[newtip_dashed] ($(refp2.south) + (0in,0in)$) -- ($(reff2.north) + (0in,0.1in)$);
  \draw[newtip_dashed] ($(refp3.south) + (0in,0in)$) -- ($(reff3.north) + (0in,0.1in)$);
  
  % cur arrows
  \draw[newline] ($(realp1.north) + (0in,0in)$) -- ($(curf1.south) + (0in,-0.1in)$);
  \draw[newline] ($(realp2.north) + (0in,0in)$) -- ($(curf2.south) + (0in,-0.1in)$);
  \draw[newline] ($(realp3.north) + (0in,0in)$) -- ($(curf3.south) + (0in,-0.1in)$);
  
  % blocks
  \node[block, anchor=north, minimum width=0.18in, minimum height=0.4in] (box1) at ($(reff1.north) + (0in,0.05in)$) {}; 
  \node[block, anchor=north, minimum width=0.18in, minimum height=0.4in] (box2) at ($(reff2.north) + (0in,0.05in)$) {}; 
  \node[block, anchor=north, minimum width=0.18in, minimum height=0.4in] (box3) at ($(reff3.north) + (0in,0.05in)$) {}; 
  
  % control
  \draw[newtip] (box1.east) -- ($(realp2.west) + (-0.05in,0in)$) node[midway,right,xshift=5pt]{$u(t_i)$} ;
  \draw[newtip] (box2.east) -- ($(realp3.west) + (-0.05in,0in)$) node[midway,right,xshift=5pt]{$u(t_{i+1})$};
  
  % time
  \node[anchor=south] (time1) at ($(refp1.north) + (0in,0in)$) {$t_0$};
  \node[anchor=south] (time2) at ($(refp2.north) + (0in,0in)$) {$t_i$};
  \node[anchor=south] (time3) at ($(refp3.north) + (0in,0in)$) {$t_{i+1}$};
  
  % text right
  \node[anchor=west] (reftext) at ($(refp3.east) + (0.1in,0in)$) {$\mcframe{\roboF}{W}{R}(t)$};
  \node[anchor=north] (refftext) at (reff3.north-|reftext.south) {$\featureSetD(t)$};
  \node[anchor=north] (curftext) at (curf3.north-|refftext.south) {$\featureSet(t)$};
  \node[anchor=north, text centered, text width=0.3in] (realptext) at (realp3.north-|curftext.south) {\centering Robot \\ Pose};
  
  \node[anchor=north] (proj1) at ($(refp1.east) + (0.35in,-0.45in)$) {\footnotesize $\camProj \circ \mcframe{h}{C}{W}(t_i)$};
  \node[anchor=north] (proj2) at ($(refp2.east) + (0.35in,-0.45in)$) {\footnotesize $\camProj \circ \mcframe{h}{C}{W}(t_{i+1})$};
  
  \node[anchor=east] (q) at ($(reff1.west) + (0in,0.2in)$) {$\pointSet^{\mc W}$};

\end{tikzpicture}

==> arxiv_submission/intro.tex <==
\section{Introduction \label{sec:Intro}}
Navigation systems with real-time needs often employ hierarchical schemes
that decompose navigation across multiple spatial and temporal scales.
Doing so permits the navigation solution to respond in real-time to novel
information gained from sensors, while being guided by the more slowly
evolving global path. At the lowest level of the hierarchy lies
trajectory tracking to realize the planned paths or synthesized
trajectories. In the absence of an absolute reference (such as GPS) and
of an accurate map of the environment, there are no external mechanisms
to support trajectory-tracking. Onboard mechanisms include odometry
through {\em proprioceptive} sensors (wheel encoders, IMUs, etc.) or
visual sensors.  Pose estimation from proprioceptive sensors is not
observable, thus visual sensors provide the best mechanism to anchor the
robot's pose estimate to external, static position references.  Indeed
visual odometry (VO) or visual SLAM (V-SLAM) solutions are essential in
these circumstances. However, they too experience drift, mostly due to the
integrated effects of measurement noise. Is it possible to do better?

The hypothesis explored in this paper is that {\em performing trajectory
tracking in the image domain reduces the sensitivity of trajectory
tracking systems reliant on VO or V-SLAM for accuracy}.  In essence, the
trajectory tracking problem is shifted from feedback in pose space to
feedback in perception space.  
Perception space approaches have several favorable properties when used
for navigation \cite{Smith2017,Smith2020}.  Shifting the representation
from being world-centric to being viewer-centric reduces computational
demands and improves run-time properties.
For trajectory tracking without reliable absolute pose information,
simplifying the feedback pathway by skipping processes that are not
relevant to--or induce sensitivities to--the local tracking task may
have positive benefits.  Using imaging sensors to control motion
relative to visual landmarks is known as {\em visual servoing}. Thus,
the objective is to explore the use of image-based visual servoing for
long-distance trajectory tracking with a stereo camera as the primary
sensor.  The technique, which we call {\em trajectory servoing}, will be
shown to have improved properties over systems reliant on VO or V-SLAM
for pose-based feedback.

%Trajectory tracking is a significant research topic in navigation systems of non-holonomic robot. Different with path following, it is required for the robot to track a spacial trajectory parameterized by time from the robot original pose, not follow a path defined only by its geometric shape without time constaints. Using visual servoing techniques, a nonholonomic robot can achieve good trajectory following without real-time robot pose information and without a known visual map of the environment. Stereo vision-based trajectory tracking could also be achieved with an on-board (VIN-)SLAM system by estimating the robot poses. But the estimation accuracy can cause higher tracking errors. It is possible to reduce the tracking error through a continuous time IBVS approach with observed features, so called trajectory servoing in this paper. 



==> arxiv_submission/longDist.tex <==
\section{Long Distance Trajectory Servoing}\label{sec:longDist}

\newcommand{\trajTimeStart}[1]{t_{#1,s}}
\newcommand{\trajTimeEnd}[1]{t_{#1,e}}
\newcommand{\featureTraj}[1]{\featureSetD_{#1} (t) |_{\trajTimeStart{#1}}^{\trajTimeEnd{#1}}}

Short-term trajectory servoing cannot extend to long trajectories due
to feature impoverishment. When moving beyond the initially visible
scene, a more comprehensive trajectory servoing system would augment
the feature pool $\featureSetD$ with new features. Likewise,
if navigation consists of multiple short distance trajectories, then
the system must have a regeneration mechanism for synthesizing entirely
new desired feature tracks for the new segment.  The overlapping needs
for these two events inform the creation of a module for feature
replenishment and trajectory extension.

% Naturally, we think about closing the loop on the image space. However, only using IBVS for trajectory tracking in an unmapped space is impossible since at least there will be a moment that all the tracked features are out of field of view (even we assume perfect tracking) and robot pose is needed to initialize a new period of IBVS. In addition, compared to PBVS, 

\begin{table*}[t]
  \vspace*{0.06in}
  \centering
  \addtolength{\tabcolsep}{-3pt}
  \begin{minipage}[t]{0.24\textwidth}
  \centering
  \caption{\textrm{Tracking ATE (cm)}\label{tb:longTrajBench}}
  \begin{tabular}{|c||ccc|}
    \hline 
    \textbf{Seq.} & PO & SLAM & TS \\ 
    \hline 
%      & \textcolor{white}{$v,\omega$} & & \\
    RU & 2.40  & 6.19   & 4.02  \\ 
    LU & 3.47  & 17.22  & 7.30  \\ 
    ST & 2.25  & 7.95   & 6.06  \\ 
    ZZ & 5.19  & 11.01  & 8.30  \\ 
    \hline 
    \textbf{Avg. ATE} & \textbf{3.33} & 10.59 & {\em 6.42} \\ 
    \hline 
  \end{tabular}
  \end{minipage}
  \begin{minipage}[t]{0.2\textwidth}
    \centering
    \caption{\textrm{Terminal Error (cm)}%
    \label{tb:longTrajTE}}
    \begin{tabular}{|c||ccc|}
    \hline 
    \textbf{Seq.} & PO & SLAM & TS \\ 
    \hline 
%      & \textcolor{white}{$v,\omega$} & & \\
    RU & 2.33  & 11.61  & 6.77  \\ 
    LU & 3.14  & 26.06  & 18.90  \\ 
    ST & 2.38  & 8.61   & 7.74  \\ 
    ZZ & 4.28  & 5.22   & 7.18  \\ 
    \hline 
    \textbf{Avg.} & \textbf{3.03} & 12.88 & \em 10.15 \\ 
    %\textbf{Std. ATE} & 0.0000 & 0.0000 & 0.0000 \\
    \hline 
    \end{tabular}
  \end{minipage}
  \begin{minipage}[t]{0.18\textwidth}
  \centering
  \caption{\textrm{Estimation ATE (cm)}%
  \label{tb:longEst}}
  \begin{tabular}{|c||cc|}
    \hline 
    \textbf{Seq.} & SLAM & TS \\ 
    \hline 
%     & \textcolor{white}{$v,\omega$} & \\
    RU & 9.15  & 8.49 \\ 
    LU & 13.68 & 11.09 \\ 
    ST & 7.00  & 7.96 \\ 
    ZZ & 12.13 & 10.37 \\ 
    \hline 
    \textbf{Avg.} & 10.49 & \textbf{\em 9.48}\\ 
    \hline 
  \end{tabular}
  \end{minipage}
  \begin{minipage}[t]{0.35\textwidth}
  \centering
  \caption{\textrm{Control Effort} \label{tb:longCost}}
  \begin{tabular}{|c||cccccc|}
    \hline 
    \textbf{Seq.} & \multicolumn{2}{c}{PO} & \multicolumn{2}{c}{SLAM} & \multicolumn{2}{c|}{TS}\\ 
    \hline 
    • & $\nu$ & $\omega$ & $\nu$ & $\omega$ & $\nu$ & $\omega$\\ 
    RU & 15.51 & 14.95 & 13.94 & 12.08 & 11.94 & 10.80 \\ 
    LU & 17.77 & 9.53  & 16.38 & 9.24  & 13.67 & 9.94 \\ 
    ST & 17.80 & 13.87 & 16.00 & 12.96 & 13.74 & 12.29 \\ 
    ZZ & 23.17 & 11.73 & 21.00 & 10.67 & 17.97 & 10.89 \\ 
    \hline 
    \textbf{Avg.} & 18.56 & 12.52 & 16.83 & 11.24 & \textbf{\em 14.33} & \textbf{\textit{10.98}}\\
    • & \multicolumn{2}{c}{31.08} & \multicolumn{2}{c}{28.07} & \multicolumn{2}{c|}{\textbf{\em 25.31}} \\
  \hline 
  \end{tabular} 
  \end{minipage}
  \addtolength{\tabcolsep}{2pt}
  \vspace*{-0.15in}
\end{table*}

%\begin{table}[h]
%  \centering
%  \begin{minipage}[t]{0.5\textwidth}
%  \centering
%  \caption{\textrm{Control Effort} \label{tb:longCost}}
%  \begin{tabular}{|c||cccccc|}
%    \hline 
%    \textbf{Seq.} & \multicolumn{2}{c}{PO} & \multicolumn{2}{c}{SLAM} & \multicolumn{2}{c|}{TS}\\ 
%    \hline 
%    • & $\nu$ & $\omega$ & $\nu$ & $\omega$ & $\nu$ & $\omega$\\ 
%    RU & 15.51 & 14.95 & 13.94 & 12.08 & 11.94 & 10.80 \\ 
%    LU & 17.77 & 9.53  & 16.38 & 9.24  & 13.67 & 9.94 \\ 
%    ST & 17.80 & 13.87 & 16.00 & 12.96 & 13.74 & 12.29 \\ 
%    ZZ & 23.17 & 11.73 & 21.00 & 10.67 & 17.97 & 10.89 \\ 
%    \hline 
%    \textbf{Avg.} & 18.56 & 12.52 & 16.83 & 11.24 & \textbf{\em 14.33} & \textbf{\textit{10.98}}\\
%    • & \multicolumn{2}{c}{31.08} & \multicolumn{2}{c}{28.07} & \multicolumn{2}{c|}{\textbf{\em 25.31}} \\
%  \hline 
%  \end{tabular} 
%  \end{minipage}
%\end{table}

\subsection{Feature Replenishment}

The number of feature correspondences $\numFeat$ in $\featureSet$ and
$\featureSetD$ indicates whether trajectory servoing can be performed
without concern.  Let the threshold $\tau_{fr}$ determine when feature
replenishment should be triggered.
Define $\featureTraj{i}$ as the $i^{\rm th}$ feature trajectory starting from
$\trajTimeStart{i}$ and ending at $\trajTimeEnd{i}$. The case $i=0$ 
represents the first feature trajectory segment generated by
\eqref{eq:featDE} for $\trajTimeStart{i}=0$, integrated up to the 
maximum time $t_{\text{end}}$ of the given trajectory.
The time varying function $\numFeat(t)$ is the actual number of feature
correspondences between $\featureSet(t)$ and $\featureSetD_i (t)$ as
the robot proceeds.

When $\numFeat(t) \ge \tau_{fr}$, the feature trajectory
$\featureSetD_i(t)$ may be used for trajectory servoing. 
When $\numFeat(t) < \tau_{fr}$, the feature replenishment process will
be triggered at the current time and noted as $\trajTimeEnd{i}$. 
The old feature trajectory $\featureTraj{i}$ is finished. 
A new feature trajectory is generated with
\begin{equation} \label{eq:trajReg}
  \featureTraj{i+1} = \camProj \circ (\roboF^*(\trajTimeEnd{i},t)
  \mcframe{\camF}{R}{C})^{-1}(\pointSet^{\mc W}(\trajTimeEnd{i})),
\end{equation}
where $\roboF^*(\trajTimeEnd{i},t)$ is the transformation between
the current robot pose and a future desired pose ($t > \trajTimeEnd{i}$) on
the trajectory.  The poses behind the robot are not included. 
The set $\pointSet^{\mc W}(\trajTimeEnd{i})$ consists of observed
points at the current time $\trajTimeEnd{i}$. 
The feature pool is augmented by these current features.  When this
regeneration step is finished, the exact time will be assigned as the
$\trajTimeStart{i+1}$.  Trajectory servoing is performed on this new
feature trajectory until the regeneration is triggered again or the
arriving at the end of the trajectory.  The process of regenerating new
feature tracks is equivalent to dividing a long trajectory into a set
of shorter segments pertaining to the generated feature trajectory
segments. 
An example of this feature replenishment is shown in Fig. \ref{fig:feat_rep}.


\begin{figure}[t]
\centering
  \vspace*{0.15in}
  \begin{tikzpicture}[inner sep=0pt, outer sep=0pt]
  \node[anchor=south west] (orig) at (0in,0in) 
    {{\includegraphics[width=0.8\columnwidth]{figs/feature_replenishment.png}}};
  
  % landmarks
  \node[anchor=west] (ti2_f) at ($(orig.west) + (-0.2in, 0.3in)$) {\footnotesize $\pointSet^{\mc W}(\trajTimeEnd{i-2})$};
  \node[anchor=west] (ti1_f) at ($(orig.west) + (0.7in, 0.3in)$) {\footnotesize $\pointSet^{\mc W}(\trajTimeEnd{i-1})$};
  \node[anchor=west] (ti_f) at ($(orig.west) + (1.4in, 0.3in)$) {\footnotesize $\pointSet^{\mc W}(\trajTimeEnd{i})$};
  
  % time
  \node[anchor=north] (ti21) at ($(ti2_f.south) + (0.05in, -0.4in)$) {\footnotesize $\trajTimeEnd{i-2}$};
  \node[anchor=north] (ti22) at ($(ti21.south) + (0in, 0in)$) {\footnotesize $\trajTimeStart{i-1}$};
  \node[anchor=north] (ti11) at ($(ti1_f.south) + (0.05in, -0.4in)$) {\footnotesize $\trajTimeEnd{i-1}$};
  \node[anchor=north] (ti12) at ($(ti11.south) + (0in, 0in)$) {\footnotesize $\trajTimeStart{i}$};
  \node[anchor=north] (ti1) at ($(ti_f.south) + (0in, -0.4in)$) {\footnotesize $\trajTimeEnd{i}$};
  \node[anchor=north] (ti2) at ($(ti1.south) + (0in, 0in)$) {\footnotesize $\trajTimeStart{i+1}$};
  
  % feature traj
  \node[anchor=north] (tib_ft) at ($(orig.west) + (0.6in, -0.45in)$) {\footnotesize $\featureTraj{i-1}$};
  \node[anchor=north] (ti_ft) at ($(orig.west) + (1.3in, -0.45in)$) {\footnotesize $\featureTraj{i}$};
  \node[anchor=north] (tin_ft) at ($(orig.west) + (2.1in, -0.45in)$) {\footnotesize $\featureTraj{i+1}$};
  
  % arrows
%  \draw[->, dashed] (ti21.north) -- ($(ti21.north) + (0in, 0.1in)$);
%  \draw[->, dashed] (ti11.north) -- ($(ti11.north) + (0in, 0.08in)$);
%  \draw[->, dashed] (ti1.north) -- ($(ti1.north) + (0in, 0.2in)$);
  
  \draw[->, very thick] (tib_ft.north) -- ($(tib_ft.north) + (0in, 0.2in)$);
  \draw[->, very thick] (ti_ft.north) -- ($(ti_ft.north) + (0in, 0.5in)$);
  \draw[->, very thick] (tin_ft.north) -- ($(tin_ft.north) + (0in, 0.2in)$);
	
  \end{tikzpicture}
  \caption{Feature replenishment process. There are three segments of feature trajectories. Stars are observed point sets at corresponding time. Each circle is the start or end time of next or this segment of feature trajectory. Three feature trajectories are generated by the feature replenishment equation \eqref{eq:trajReg}. \label{fig:feat_rep}}
  \vspace*{-1em}
\end{figure}

During navigation, \eqref{eq:trajReg} requires the current robot pose
relative to the initial pose to be known.  In the absence of an
absolute reference or position measurement system, the only option
available is to use the estimated robot pose from V-SLAM, or some
equivalent process. 
Although there are some drawbacks to relying on V-SLAM, it attempts to
keep pose estimation as accurate as possible over long periods through
feature mapping, bundle adjustment, loop closure, etc.. 
To further couple V-SLAM and trajectory servoing, we design a multi-loop
scheme, see Fig. \ref{fig:BlockTS}. The inner loop is governed by
trajectory servoing with V-SLAM tracked features. The V-SLAM estimated
pose will only be explicitly used in the outer loop when performing
feature replenishment. In this way, the inner visual feedback loop will
not be affected by the uncertainty from pose estimation. Plus the outer
loop will only be activated when starting a new feature replenishment; 
and since the visual information is received, fused, and optimized
with an IMU, it generates a robot pose that is more reliable than the raw
poses used in the inner loop of V-SLAM pose based control (shown in Fig.
\ref{fig:posebasedcontrol}).
However, relying on V-SLAM still introduces measurement error or drift,
which means that long-term trajectory servoing along an absolute,
desired trajectory will accrue error.

\tikzset{global scale/.style={
    scale=#1,
    every node/.append style={scale=#1}
  }
}
\begin {figure}
\vspace*{-1em}
\centering
%\begin{adjustbox}{width=\textwidth}
\begin{tikzpicture}[global scale = 0.7]
% Sum shape
\node [draw,
    fill=Goldenrod,
    minimum width=1.5cm,
    minimum height=1cm,
    text width=2.5cm,
    text centered
]  (FG) at (0,0) {\centering Feature \\ Replenishment};

\node[draw,
    circle,
    minimum size=0.6cm,
    fill=Rhodamine!50,
    right=0.5cm of FG
] (sum){};
 
\draw (sum.north east) -- (sum.south west)
    (sum.north west) -- (sum.south east);
 
\draw (sum.north east) -- (sum.south west)
(sum.north west) -- (sum.south east);
 
\node[left=-1pt] at (sum.center){\tiny $+$};
\node[below] at (sum.center){\tiny $-$};
 
% Controller
\node [draw,
    fill=Goldenrod,
    minimum width=1.5cm,
    minimum height=1cm,
    text width=2cm,
    text centered,
    right=0.5cm of sum
]  (controller) {\centering Trajectory \\ Servoing};
 
% System H(s)
\node [draw,
    fill=SpringGreen, 
    minimum width=1.5cm,
    minimum height=1cm,
    right=0.7cm of controller
] (system) {Plant};
 
% Sensor block
\node [draw,
    fill=SeaGreen, 
    minimum width=1.5cm,
    minimum height=1cm,
    below right= 0.4cm and -0.8cm of controller
]  (sensor) {Tracked Features};

\node [draw,
    fill=SeaGreen, 
    minimum width=1.5cm,
    minimum height=1cm,
    below right= 1.5cm and -1.1cm of controller
]  (SLAM) {V-SLAM Pose};
 
% Arrows with text label
\draw[-stealth] (sum.east) -- (controller.west)
    node[midway,above]{$e$};
 
\draw[-stealth] (controller.east) -- (system.west) 
    node[midway,above]{$\dot{\featSetV},u$};
    
\draw[-stealth] ($(controller.north) + (0in, 0.3in)$) -- (controller.north)
    node[midway,right]{$u^*$};
 
\draw[-stealth] (system.east) -- ++ (1.25,0) 
    node[midway](output){}node[midway,above]{$\featSetV,\mcframe{\roboF}{W}{R}$};
 
\draw[-stealth] (output.center) |- (sensor.east);
 
\draw[-stealth] (sensor.west) -| (sum.south) 
    node[near end,left]{$\hat{\featSetV}$};
 
\draw [-stealth](FG) --(sum.west) 
    node[midway,above]{$\featSetDV$};
    
\draw [-stealth] ($(FG.west) + (-1.5,0)$) -- (FG.west)
    node[midway,above]{Ref Traj};
    
     
\draw[-stealth] (output.center) |- (SLAM.east);
 
\draw[-stealth] (SLAM.west) -| (FG.south) 
    node[near end,left]{$\hat{{\roboF}}^{\mc{W}}_{\mc{R}}$};
\end{tikzpicture}
\caption{Block Diagram for long-term Trajectory Servoing \label{fig:BlockTS}}

%\end{adjustbox}
\end{figure}



==> arxiv_submission/longExp.tex <==
%\color{orange}
%A standard navigation system usually involves environment perception,
%path planning and low level control.  Many prior works have introduced
%SLAM system to localize robot and build map of the unknown environment.
%Then path planning is possible to perform based on the combination
%known map and the sensed map. Low level control that follows the
%planned path can be achieved by pose-based trajectory tracking
%approaches with the online estimated robot poses from SLAM.  However,
%the tracking accuracy largely depends on the localization.  The biased
%or jumped localization will lead to the inaccuracy of tracking.
%Therefore, it is necessary to design a new tracking system that does
%not explicitly depend on the localization and still have a high
%tracking accuracy.  In this way, we can have the best probability to
%avoid collisions when following the valid planned path.
%
%In addition, due to the limited FoV and trusted sensing range of the camera, 
%the initial feature set $\featureSetD(0)$ can only be transformed to the poses 
%of trajectory within a limited range. 
%Also, because of the feature impoverishment in tracking, the number of 
%correspondence features between $\featureSet$ and $\featureSetD$ may decrease to 0.
%Therefore, the trajectory servoing can only be performed on a 
%short term trajectory.  
%In this section, we firstly discuss and present the experiment results of 
%this local trajectory servoing.
%\color{black}

\begin{figure}[t]
\centering
  %\vspace*{-0.125in}
  \begin{tikzpicture}[inner sep=0pt, outer sep=0pt]
  \node[anchor=south west] (RU) at (0in,0in) 
    {{\includegraphics[width=35pt]{figs/ICRA2021Figs/LongFigs/turn.png}}};
  \node[anchor=south west,xshift=10pt] (LU) at (RU.south east)
    {\includegraphics[width=35pt]{figs/ICRA2021Figs/LongFigs/twocircle.png}};
  \node[anchor=south west,xshift=10pt] (ST) at (LU.south east)
    {\includegraphics[width=45pt]{figs/ICRA2021Figs/LongFigs/loop.png}};
  \node[anchor=south west,xshift=10pt] (ZZ) at (ST.south east)
    {\includegraphics[width=35pt]{figs/ICRA2021Figs/LongFigs/zigzag.png}};

  \node[anchor=north] at (RU.south) {\footnotesize RU};
  \node[anchor=north] at (LU.south) {\footnotesize LU};
  \node[anchor=north] at (ST.south) {\footnotesize ST};
  \node[anchor=north] at (ZZ.south) {\footnotesize ZZ};
  \end{tikzpicture}
  \vspace*{-0.5em}
  \caption{Long-distance trajectories\label{fig:long_trajs}}
%\end{figure}
%\begin{figure}[t]
  \vspace*{0.2em}
  \centering
  %\includegraphics[scale=0.13,clip=true,trim=0in 3in 0in 1.25in]{figs/longbox_update.png}
%  \includegraphics[scale=0.15]{figs/longbox_update.png}
  {\includegraphics[width=2.5in,clip=true,trim=0in 0in 0in 0in]{figs/longbox_fixed.png}}
  \vspace*{-0.5em}
  \caption{Long trajectory benchmarking results\label{fig:longbench}}
  \vspace*{-1em}
\end{figure}

\subsection{Experiments and Results\label{sec:longDist_exp}}

This section modifies the experiments in \S\ref{sec:shortDist_exp} to
involve longer trajectories that will trigger feature replenishment and
synthesize new feature trajectory segments. The set of trajectories to
track is depicted in Fig. \ref{fig:long_trajs}. They are denoted as
right u-turn (RU), left u-turn (LU), straight+turn (ST), and zig-zag
(ZZ). Each trajectory is longer than 20m. 
Testing and evaluation follows as before (minus VS+).

\subsubsection{Results and Analysis}
Fig. \ref{fig:longbench} consists of boxplots of the
translation-only trajectory tracking ATE for the template
trajectories. As hypothesized, the error over longer trajectories is
affected by the need to use SLAM pose estimates for regeneration. The PO
method outperforms TS, but TS still operates better than SLAM.
However, it appears that in the one case where the SLAM system
performed the worst, the TS approach had better performance. The
tabulated results in Tab. \ref{tb:longTrajBench} and \ref{tb:longTrajTE} 
indicates that on
average the TS approach improved over SLAM by 39\% and 21\% in terms of tracking
error and terminal error. 
What is interesting is that the estimation ATE of both systems is
comparable (Tab.~\ref{tb:longEst}), which indicates that trajectory
servoing may have better closed-loop noise rejection properties by
working directly in image-space instead of using inferred pose estimates
from the SLAM estimator. Tab. \ref{tb:longCost} suggests that control
efforts of both $\nu$ and $\omega$ are the lowest. The combined control
effort of TS is reduced 19\% and 10\% from PO and SLAM. That TS may change
the performance vs. cost trade-off curves should be studied further. 

\subsection{Navigation with online path planning}


\begin{figure}[t]
	\centering
	\begin{tikzpicture}[inner sep=0pt,outer sep=0pt]
	\node[anchor=south west, xshift=10pt] (gt) at (0in,0in)
    {\includegraphics[width=1in]{figs/nav_demo_gt.png}};
    \node[anchor=south west, xshift=10pt] (vs) at (gt.south east)
    {\includegraphics[width=1in]{figs/nav_demo_vs_terminals_new.png}};
    \node[anchor=south west, xshift=10pt] (slam) at (vs.south east)
    {\includegraphics[width=1in]{figs/nav_demo_slam.png}};
    
    \node[anchor=north west,fill=white,inner sep=2pt,xshift=-1pt,yshift=0pt] 
      at (gt.north west) {\small (a)};
    \node[anchor=north west,fill=white,inner sep=2pt,xshift=-1pt,yshift=0pt] 
      at (vs.north west) 
    {\small (b)};
    \node[anchor=north west,fill=white,inner sep=2pt,xshift=-1pt,yshift=0pt] 
      at (slam.north west) {\small (c)};
    
  \end{tikzpicture}
 	\caption{Navigation with global planning. Blue point is the robot starting position. Orange points are 6 goal points for navigation. In each figure, green is the collision-free global path. Red is the real robot trajectory overlaying on the green trajectory. The figures show successful navigation examples of the same goal point with three different controllers. (a) Pose-based trajectory tracking with perfect odometry. (b) Vision-based trajectory servoing. (c) Pose-based trajectory tracking with estimated poses from V-SLAM. It can be observed that the red trajectory has less deviations from the green trajectory with TS (b) than SLAM (c).
	\label{fig:nav_demo}}
\vspace*{-0.5em}
\end{figure}


%\begin{figure}[hbtp]
%	\centering
%	\includegraphics[scale=0.05]{figs/nav_demo_large.png}
%	\caption{Trajectory servoing with the online path planning in the same environment. Green is the collision-free global path. Red is the real robot trajectory. The robot starts from the bottom and ends at the top point.}
%	\label{fig:nav_demo}
%\end{figure}

To show how trajectory servoing works for a navigation task, we move the
environment down to the ground and create a 2D occupancy map.
Given a goal, the global planner identifies a feasible collision-free
path from the map.  The online global path is used for the robot to
apply trajectory servoing. 
The full system in Fig. \ref{fig:system_flowchart} is used.
Fig. \ref{fig:nav_demo} shows one successful navigation task for three tracking 
methods. 
The robot starts from the blue point, and ends at 
6 different positions, marked as orange points. 
The average ATE for PO, SLAM and TS are 1.31cm, 7.39cm and 7.30cm. 
And the average terminal errors are 1.46cm, 14.49cm and 13.13cm.
Trajectory servoing, enabled by V-SLAM, has better performance than
using V-SLAM for pose-based feedback. The smaller performance gap
between TS and SLAM for these navigation tasks requires further
investigation. Per Tables \ref{tb:shortEst} and \ref{tb:longEst}, it
appears to be dependent on SLAM estimation error, as the gap is close to
the estimation gap ($\sim$10\%). There may be a mechanism to better
estimate motion from the initial pose to the terminal pose of a
trajectory segment, which might involve more tightly coupling the short
distance module with the SLAM module (see
Fig.~\ref{fig:system_flowchart}).


==> arxiv_submission/review.tex <==
\subsection{Image-Based Visual Servoing Rate Equations\label{sec:ibvs}}

The core algorithm builds on IBVS \cite{538972}, thus
this section covers IBVS with an emphasis on how it directly relates the
velocity of image features to the robot velocities via the image Jacobian
\cite{4015997,4141039}. These equations will inform the trajectory
tracking problem under non-holonomic robot motion. We use the more
modern notation from geometric mechanics \cite{MLS} since it provides 
equations that better connect to contemporary geometric control
and SLAM formulations for moving rigid bodies.

%\toedit{
%Image based visual servoing (IBVS) is widely applied in trajectory
%tracking of manipulators. It shows that the velocity of features could be
%directly related to the robot velocities using image jacobian. So we can
%borrow this idea into our navigation process. Cite book notation comes
%from.}

\newcommand{\roboF}{g}
\newcommand{\roboBV}{\xi_u}
\newcommand{\camF}{h}
\newcommand{\camBV}{\zeta_u}
\newcommand{\camProj}{H}
\newcommand{\camPt}{r}

\newcommand{\imJac}{{L}}
\newcommand{\imJacV}{\boldsymbol{L}}

\newcommand{\geoJac}{{G}}

\newcommand{\numFeat}{n_{\text{F}}}


\newcommand{\pose}{\boldsymbol{P}}
\newcommand{\control}{\boldsymbol{u}}
\newcommand{\transCR}{^C\boldsymbol{T}_{R}}
\newcommand{\transCRv}{^C\boldsymbol{T}_{R,v}}
\newcommand{\transCRw}{^C\boldsymbol{T}_{R,\omega}}


\newcommand{\pointSet}{\boldsymbol{Q}}
\newcommand{\pointSetV}{\boldsymbol{q}}

\newcommand{\featureSet}{\boldsymbol{S}}
\newcommand{\featSetV}{\boldsymbol{s}}
\newcommand{\featSetDV}{\boldsymbol{s}^*}
\newcommand{\featSetDVdot}{\dot{\boldsymbol{s}}^*}
\newcommand{\featureSetA}{\boldsymbol{S}_a}
\newcommand{\featureSetD}{\boldsymbol{S}^*}
\newcommand{\featureSetDA}{\boldsymbol{S}_a^*}

\newcommand{\error}{\boldsymbol{e}}
\newcommand{\errorSet}{\boldsymbol{E}}

\newcommand{\imageJacobian}{\boldsymbol{L}}

\newcommand{\imageJacobiani}{\boldsymbol{L}_{S_i}}
\newcommand{\imageJacobianv}{\boldsymbol{L}_{S,v}}
\newcommand{\imageJacobianw}{\boldsymbol{L}_{S,\omega}}
\newcommand{\transFeature}{g}
\newcommand{\homo}{H}

%\begin{figure}[h]
%  \centering
%  \includegraphics[height=1.75in]{figs/model_of_non-holonomic_robot.png}
%  \caption{\color{red}Model of non-holonomic mobile robot with camera.
%  \label{fig:robot_model}}
%\end{figure}

%============================ Motion Models ============================

\subsubsection{Non-Holonomic Robot and Camera Kinematic Models}
%In basic IBVS problems, the two major procedures are first establish the linear map $\geoJac$ from control velocity space to the camera velocity, which is called Geometric Jacobian and the linear map $\imJac$ from camera velocity space to feature velocity space. In a kinematic Hilare robot model where the pose state
%$\mcframe{\roboF}{W}{R} \in SE(2)$ evolves under the control $u = [\nu, \omega]^T$, we have: $\geoJac: \Real^2\rightarrow \Real^3$ and $\imJac: \Real^3\rightarrow \Real^2$.
%
%We assume $\camBV \in \LA{se}(2)$ is the camera velocity twist in camera frame and $\roboBV \in \LA{se}(2)$is the robot velocity twist in robot frame. They are related by the formula:
%\begin{eqnarray}
%\camBV=\Ad^{-1}_{\mcframe{h}{R}{C}}\cdot\roboBV=\underbrace{\Ad^{-1}_{\mcframe{h}{R}{C}}\cdot\begin{bmatrix} 1 & 0 \\ 0 & 0 \\ 0 & 1 \end{bmatrix}}_{\geoJac}\cdot
%\begin{bmatrix} \nu \\ \omega \end{bmatrix}
%=\geoJac \cdot u
%\end{eqnarray}
%Then we write the dynamics of the feature on the image space $\camPt\in\Real^{2}$ with the coordinates of feature in the camera frame $\pointSetV{^{\mc C}}$, the image Jacobian $\imJac$ and camera velocity twist $\roboBV \in \LA{se}(2)$:
%\begin{eqnarray}
%\dot \camPt = \imJac(q^{\mc C}) \camBV=\underbrace{\imJac(q^{\mc C})\cdot\geoJac}_{\imJac_u}\cdot u=\imJac_u(q^{\mc C}; \mcframe{h}{R}{C})\cdot u
%\end{eqnarray}
%We see the Geometrical Jacobian is absorbed into the Image Jacobian and form a new image Jacobian $\imJac_u(q^{\mc C}; \mcframe{h}{R}{C})$ that directly relates the feature dynamics to robot dynamics.
Let the motion model of the robot be a kinematic Hilare robot model
where the pose state
$\mcframe{\roboF}{W}{R} \in SE(2)$ evolves under the control $u = [\nu,
\omega]^T$ as
\begin{equation} \label{eq:roboDE}
  \mcframe{\dot \roboF}{W}{R} 
    = \mcframe{\roboF}{W}{R} 
      \cdot \begin{bmatrix} 1 & 0 \\ 0 & 0 \\ 0 & 1 \end{bmatrix}
      \begin{bmatrix} \nu \\ \omega \end{bmatrix}
    = \mcframe{\roboF}{W}{R} \cdot \roboBV,
\end{equation}
for $\nu$ a forward linear velocity and $\omega$ an angular velocity, and 
$\roboBV \in \LA{se}(2)$.
The state is the robot frame $\mc{R}$ relative to the world frame
$\mc{W}$. The camera frame $\mc{C}$ is presumed to be described as 
$\mcframe{\camF}{R}{C}$ relative to the robot frame. Consequently, camera
kinematics relative to the world frame are
\begin{equation} \label{eq:camDE}
  \mcframe{\dot \camF}{W}{C} 
    = \mcframe{\roboF}{W}{R} \cdot \mcframe{\camF}{R}{C}
      \cdot \Ad^{-1}_{\mcframe{h}{R}{C}} \cdot 
      \begin{bmatrix} 1 & 0 \\ 0 & 0 \\ 0 & 1 \end{bmatrix}
      \begin{bmatrix} \nu \\ \omega \end{bmatrix}.
    = \mcframe{\roboF}{W}{R} \cdot \mcframe{\camF}{R}{C}
      \cdot \camBV
\end{equation}
with $\camBV \in \LA{se}(2)$.
%Let the camera projection equations for points specified in the world
%frame be given by $\camProj:\Real^3 \rightarrow \Real^2$. Then
Now, let the camera projection equations be given by the function
$\camProj:\Real^3 \rightarrow \Real^2$ such that a point $q^{\mc{W}}$
projects to the camera point $\camPt = \camProj \circ \mcframe{\camF}{C}{W}
(q^{\mc W})$. Under camera motion, the differential equation relating
the projected point to the camera velocity is
\begin{equation} \label{eq:camDEsimp}
  \dot \camPt = \text{D}\camProj(q^{\mc C}) \cdot
    \left( \camBV \cdot q^{\mc C} \right),
\end{equation}
where the point $q$ is presumed to be static, i.e., $\dot q = 0$, and
$q^{\mc C} = \mcframe{\camF}{C}{W} q^{\mc W}$, and $\text{D}$ is the
differential operator. 
Since the operation 
$\xi \cdot q$ is linear for $\xi \in \LA{se}(2)$, $q \in \Real^3$, it can
be written as a matrix-vector product $M(q) \xi$ leading to,
\begin{equation} \label{eq:camPtDot}
  \dot \camPt = \text{D}\camProj(q^{\mc C}) \cdot M(q^{\mc C}) \camBV 
    = \imJac(q^{\mc C}) \camBV.
\end{equation}
where $\imJac:\Real^3 \times \LA{se}(2)$ is the Image Jacobian. Given the point and projection pair
$(q,\camPt) \in \Real^3 \times \Real^2$, $\imJac$ works out to be
\begin{equation} \label{eq:imJac}
  \imJac(q) = \imJac(q,r) = 
    \begin{bmatrix*}
      - \frac{f}{q^3} & 0 
      %& \frac{r^1}{q^3} & \frac{r^1 r^2}{f} & -\frac{f^2+(r^1)^2}{f} 
      & r^2 \\[1pt]
      0 & -\frac{f}{q^3} 
      %& \frac{r^2}{q^3} & \frac{f^2+(r^2)^2}{f} & -\frac{r^1 r^2}{f} 
      & -r^1
    \end{bmatrix*},
\end{equation}
where $f$ is the focal length. 
Recall that $r = \camProj(q)$. Re-expressing it as a function of $(q,r)$
simplifies its written form, and exposes what information is available
from the image directly $r \in \Real^2$ and what additional information
must be known to compute it: coordinate $q^3$ from $q^{\mc C} \in
\Real^3$ in the camera frame, which is also called depth. 
With a stereo camera, the depth value is triangulated. The next section
will use these equations for image-based trajectory tracking.




%\color{red}
%The trajectory servoing system we proposed hits all the topics we have mentioned before: visual servo, outlier rejection and statistical benchmarking. We will show that the SLAM based trajectory servoing performs better than other controllers, and is capable for long-term trajectory navigation. The contributions are:
%
%1) Given a trajectory in the Cartesian space, we designed an feature-based trajectory tracking (i.e. trajectory servoing) system for non-holonomic mobile robot (turtlebot). The feature points are obtained from the stereo-based GF ORB SLAM \cite{gf_orb_slam}. Motion model (especially image jacobian) is derived to fit in the system.
%
%%2) Built an model to describe how the uncertainty of the image features were propagated and affect the tracking. More importantly, used a generalized least square method to weigh the contributions of each feature instead of directly cutting off some features. Matlab simulation is given here to show our model and the result of the improved controller.
%
%2) Due to the limited Field-of-View and the maximum range of camera sensor, the approach is extended to the long-term navigation. When the number of useful features is too low, a new feature trajectory is regenerated from the original long trajectory by querying the estimated robot pose from the VI-SLAM system. In this way, the long-term trajectory tracking is achieved.
%
%3) We also developed a benchmarking platform to compare different configurations statistically. The configurations include different trajectory tracking approaches, such as pose-based methods with different robot pose settings, visual-based method (i.e. trajectory servoing). The comparison results indicate the improvement of tracking accuracy with trajectory servoing.
%\color{black}

\begin{figure}[t]
  \vspace*{0.06in}
  \centering
  \includegraphics[width=0.9\columnwidth]{figs/framework.png}
%  \scalebox{0.6}{\input{figs/trajservo_process.tex}}
  \caption{A trajectory servoing system has two major components. 
  One steers the robot to track short paths, while the other
  ensures the sufficiency of features to use by querying a SLAM module.
  \label{fig:system_flowchart}}
\end{figure}

%Fig. \ref{fig:system_flowchart} is the entire navigation system to
%represent how trajectory servoing works with long-term navigation.  The
%combination of VI-SLAM and trajectory servoing gives a full solution to
%this task.




==> arxiv_submission/shortDist.tex <==
\section{Trajectory Servoing}\label{sec:shortDist}

\subsection{Contributions \label{sec:BG_cont}}

The system described in this paper blends visual servoing, SLAM, and
basic concepts from VTR to enable trajectory tracking of feasible paths
by a mobile robot in unknown environments with sufficient visual
texture. We call this combination of methods {\em trajectory servoing}
because the objective is to perform long-term trajectory tracking using
visual servoing techniques. What enables this objective to be met is a
stereo visual SLAM system \cite{8964284}, which ties the desired
trajectory to the image information.

The algorithmic components and information flow of a trajectory
servoing system are depicted in Fig.~\ref{fig:system_flowchart}, and
consist of two major components.  The first one, described in 
\S\ref{sec:shortDist}, is a trajectory servoing system for a set of
world points and specified trajectory.  These points are obtained from
the V-SLAM system as well as tracked over time.  It is capable of
guiding a mobile robot along short paths. The second component,
described in \S\ref{sec:longDist}, supervises the core trajectory
servoing system and confirms that it always has sufficient features from
the feature pool to operate.  Should this quantity dip too low, it
queries the V-SLAM module for additional features and builds new feature
tracks. 

Both \S\ref{sec:shortDist} and \S\ref{sec:longDist} include
benchmarking and evaluation experiments quantifying the performance of
the core trajectory servoing system for short paths and the
entire system for long paths. Trajectory servoing is pretty
unique in that short-term trajectories can be tracked as well as
pose-based feedback control with access to perfect odometry. Though
long-term accuracy is undermined by the reliance on SLAM, 
trajectory servoing minimizes the reliance and exhibits less
sensitivity to estimation error than pose feedback methods.

%It then describes how IBVS is integrated into the trajectory
%tracking component of a standard navigation pipeline with a VO or V-SLAM
%component to form a {\em{trajectory servoing}} system. 
%Simple short distance trajectory tracking experiments quantify
%the performance improvements that result from a short circuited
%closed-loop pathway for trajectory tracking.



%================================= IBVS ================================

\subsection{Trajectory Servoing}

Pose-based feedback control is generally used in trajectory tracking. 
In the absence of global position knowledge, V-SLAM system provides the pose
estimates needed for feedback.
Tracking performance will largely depend on localization accuracy since
the V-SLAM system serves as an observer of robot pose in the feedback
loop.  Fig. \ref{fig:posebasedcontrol} shows the block diagram of the
typical V-SLAM pose-based control architecture.  Pose estimation is
sensitive to image measurements.  Any uncertainty (e.g. IMU bias, camera
noise, calibration error, etc.) will accumulate
\cite{Liu2014NavigationalDA}, immediately affect the feedback loop and
further affect the control result.  In addition, high visual processing
latency will cause lower estimation accuracy due to late correction of
raw IMU data \cite{zhao2020closednav}.
%It has been recognized that IBVS is remarkably more robust to such noise or disturbance than PBVS\cite{4015997} which also shares the similar localization process vulnerable to uncertainty\cite{VSwheel} as VI-SLAM.
To overcome these shortcomings, we design a mobile robot tracking method
that bypasses pose feedback and provides feedback control directly
through the image space.
%In addition, the control rate of this control loop is fast enough($\approx 100$HZ) such that it is high likely no correction and fusion of the raw IMU data is applied in this period from the visual latency\cite{9197003}, which will further do harm to the system. 
%Therefore, we are reluctant to use SLAM pose in the feedback loop of trajectory tracking.

\tikzset{global scale/.style={
    scale=#1,
    every node/.append style={scale=#1}
  }
}
\begin{figure}[t]
\centering
\begin{tikzpicture}[global scale = 0.7]
% Sum shape
\node[draw,
    circle,
    minimum size=0.6cm,
    fill=Rhodamine!50
] (sum) at (0,0){};
 
\draw (sum.north east) -- (sum.south west)
    (sum.north west) -- (sum.south east);
 
\draw (sum.north east) -- (sum.south west)
(sum.north west) -- (sum.south east);
 
\node[left=-1pt] at (sum.center){\tiny $+$};
\node[below] at (sum.center){\tiny $-$};
 
% Controller
\node [draw,
    fill=Goldenrod,
    minimum width=2cm,
    minimum height=1.2cm,
    right=1cm of sum
]  (controller) {Controller};
 
% System H(s)
\node [draw,
    fill=SpringGreen, 
    minimum width=2cm, 
    minimum height=1.2cm,
    right=1.5cm of controller
] (system) {Plant};
 
% Sensor block
\node [draw,
    fill=SeaGreen, 
    minimum width=2cm, 
    minimum height=1.2cm, 
    below right= 0.4cm and -0.25cm of controller
]  (sensor) {V-SLAM Pose};
 
% Arrows with text label
\draw[-stealth] (sum.east) -- (controller.west)
    node[midway,above]{$e$};
    
\draw[-stealth] ($(controller.north) + (0in, 0.3in)$) -- (controller.north)
    node[midway,right]{$u^*$};
 
\draw[-stealth] (controller.east) -- (system.west) 
    node[midway,above]{$u$};
 
\draw[-stealth] (system.east) -- ++ (1.25,0) 
    node[midway](output){}node[midway,above]{$\mcframe{\roboF}{W}{R}$};
 
\draw[-stealth] (output.center) |- (sensor.east);
 
\draw[-stealth] (sensor.west) -| (sum.south) 
    node[near end,left]{$\hat{{\roboF}}^{\mc{W}}_{\mc{R}}$};
 
\draw[-stealth] ($(sum.west) + (-1,0)$) -- (sum.west) 
    node[midway,above]{$\mcframe{\roboF}{W,*}{R}$};
\end{tikzpicture}
\caption{Block Diagram for V-SLAM Posed Based Control}
\label{fig:posebasedcontrol}
\end{figure}

The standard IBVS equations presented in \S\ref{sec:ibvs} typically
apply to tracked features with known static positions in the world
(relative to some frame attached to these positions). 
As described in \S \ref{sec:BG_vtr} and \S \ref{sec:BG_vs}, a visual map
or visible targets are usually necessary.
The prerequisites needed for stable tracking and depth recovery of
features are major challenges regarding the use of visual servoing 
in unknown environments.  Fortunately, they are all possible to
meet based on information and modules available within the software
stack of an autonomous mobile robot. This section describes the basic
{\em trajectory servoing} implementation and describes how to build a
solution that satisfies the prerequisites. It focuses on short-term
navigation where sufficient image features remain within the field of
view for the entire trajectory.

Trajectory servoing requirements condense down to the following: 
1. A set of image points, $\featureSet^*(t_0)$, with known (relative) 
positions; 
2. A given trajectory and control signal for the robot starting at the
robot's current pose or nearby, $\mcframe{\roboF}{W}{R}(t_0)$; and 
3. The ability to index and associate the image points across future
image measurements, $\featureSet^*(t) \leftrightarrow \featureSet(t)$,
when tracking the trajectory.  The trajectory servoing process and
variables are depicted in Fig.  \ref{fig:trajservo_demo}.  The autonomy
modules contributing this information are the navigation and V-SLAM
stacks. The navigation stack generates a trajectory to follow. 
An indirect, feature-based V-SLAM stack will keep track of points in the
local environment and link them to previously observed visual features
while also estimating their actual position relative to the robot.  

\begin{figure}
  \hspace{-0.3in}
  \centering
  \begin{tikzpicture}[inner sep=0pt, outer sep=0pt, auto, >=latex]
  \node[anchor=south west] (fig) at (0,0)
    	{{\scalebox{1}{\input{figs/trajservo_demo.tex}}}};
  \end{tikzpicture}
  \caption{Trajectory servoing process. Matches from
  $\featureSet^*$ to $\featureSet$ define the control $u$, where
  $\featureSet^*(t)$ is defined by the desired trajectory.\label{fig:trajservo_demo}}
\end{figure}

\subsubsection{Trajectory and control signals}
%For the intents of this section, we will 
Define $\featureSet = \set{\camPt_i}_{1}^{\numFeat} \subset \Real^2$ as a set of image points in the current camera image, sourced from the set $\pointSet = \set{q_i^{\mc W}}_{1}^{\numFeat} \subset \Real^3$ 
of points in the world frame.  Suppose that the robot should attain a future pose given by $\roboF^*$, for which the points in $\pointSet$ will project to the image coordinates $\featureSetD = \camProj \circ
(\roboF^* \mcframe{\camF}{R}{C})^{-1}(\pointSet)$. For simplicity,
ignore field of view issues and occlusions between points. Their effect
would be such that only a subset of the points in $\pointSet$ would
contribute to visual servoing.

Assume that a specific short-duration path has been established as the
one to follow, and has been converted into a path relative to the
robot's local frame. It either contains the current robot pose in it, or
has a nearby pose. Contemporary navigation stacks have a means to
synthesize both a time varying trajectory and an associated control
signal from the paths. Here, we apply a standard trajectory tracking
controller \cite{NITraj}.  to generate $\roboBV^*(t)$ and
$\mcframe{\roboF}{W,*}{R}(t)$ by forward simulating \eqref{eq:roboDE};
note that $\roboBV^*$ contains the linear velocity $\nu^*$ and angular
velocity $\omega^*$. Some navigation stacks use optimal control
synthesis to build the trajectory. %e.g. near identity 
Either way, the generated trajectory is achievable by the robot.

In the time-varying trajectory tracking case, we assume that a trajectory reference $\mcframe{\camF}{W}{C}(t)$ exists along with a control signal $u^*(t)$ satisfying \eqref{eq:camDE}. It would typically be derived from
a robot trajectory reference $\mcframe{\roboF}{W}{R}(t)$ and control signal $u^*(t)$ satisfying \eqref{eq:roboDE}. Using those time-varying functions, the equations in \eqref{eq:camDE} are solved to obtain the image coordinate trajectories. Written in short-hand to expose only the main variables, the forward integrated feature trajectory $\featureSetD$ is:
\begin{equation}  \label{eq:featDE}
\begin{split}
  \dot \featureSetD & = \imJac \circ \mcframe{h}{C}{W}(t)(\pointSet^{\mc W}) \cdot
    \zeta_{u^*(t)}, \ \text{with} \\
    \featureSetD(0) & = \camProj \circ \mcframe{h}{C}{W}(0)(\pointSet^{\mc W}).
\end{split}
\end{equation}
It will lead to a realizable visual servoing problem where $\nu^*$, $\omega^*$, and $\featureSetD(t)$ are consistent with each other. The equations will require converting the reference robot trajectory to a camera trajectory $\mcframe{\camF}{W,*}{C}(t)$ using \raisebox{1pt}{$\Ad^{-1}_{\mcframe{h}{R}{C}}$}.
\vspace{4pt}
\subsubsection{Features and feature paths\label{FeatPaths}}
The V-SLAM module provides a pool of visible features with known relative position for the current stereo frame, plus a means to assess future visibility if desired. Taking this pool to define the feature set $\featureSetD(0)$ gives the final piece of information
needed to forward integrate \eqref{eq:featDE} and generate feature
trajectories $\featureSetD(t)$ in the left camera frame. This process
acts like a short-term teach and repeat feature trajectory planner but
is {\em simulate} and repeat, for on-the-fly generation of the repeat data. 

A less involved module could be used besides a fully realized V-SLAM system, however doing so would require creating many of the fundamental building blocks of an indirect, feature-based V-SLAM system. 
%Components needed include feature detection, feature matching, and map
%point estimation.  Map point estimation could be removed, but at the
%consequence of introduction error in the map point depth estimation
%from individual stereo measurement. 
Given the availability of strong performing open-source, real-time V-SLAM methods, there is little need to create a custom module. 
In addition, an extra benefit to tracked features through V-SLAM system
is that a feature map is maintained to retrieve same reappeared
features. As will be shown, this significantly improves the average
lifetime of features, especially compared to a simple frame by frame
tracking system without the feature map. 

After the V-SLAM feature tracking process, we are already working with this feasible set whereby the indexed elements in $\featureSet$ correspond exactly to their counterpart in $\featureSetD$ with the same index, i.e., the sets are {\em in correspondence}.
\subsubsection{Trajectory Servoing Control}
Define the error to be $\errorSet = \featureSet - \featureSetD$ where
elements with matched indices are subtracted. The error dynamics of the
points are:
\begin{equation} \label{eq:ErrorSetDE}
  \errorSet = \dot \featureSet - \dot \featureSetD = 
    \imJac_u(\mcframe{\camF}{C}{W}(\pointSet), \featureSet; \mcframe{h}{R}{C}) \cdot u - \dot \featureSetD
\end{equation}
where we apply the same argument adjustment as in \eqref{eq:imJac} so
that dependence is on image features then point coordinates as needed.
Further, functions or operations applied to indexed sets will return an
indexed set whose elements correspond to the input elements from the
input indexed set. Since the desired image coordinates $\featureSetD$
are not with respect to a static goal pose but a dynamic feature
trajectory, $\dot \featureSetD \neq 0$, see \eqref{eq:featDE}.
Define $\error$, $\featSetV$, $\featSetDV$, and $\imJacV$ to be the
vectorized versions
of $\errorSet$, $\featureSet$, $\featureSetD$ and $\imJac$. Then,
\begin{equation} \label{eq:errorDE}
  \dot \error =
  \imJacV(\mcframe{\camF}{C}{W}(\pointSetV),\featSetV;\mcframe{h}{R}{C}) \cdot u
    - \featSetDVdot
\end{equation}
is an overdetermined set of equations for $u$ when $\numFeat > 2$.
Removing the functional dependence and breaking apart the different
control contributions, the objective is to satisfy,
\begin{equation} \label{eq:IBVSw}
  \dot \error = \imJacV \cdot u-\featSetDVdot = \imJacV^1 \nu + \imJacV^2 \omega -\featSetDVdot
              = -\lambda \error.
\end{equation}
A solution is to define,
\begin{equation} \label{eq:vStEq}
  \omega = {\of{\imJacV^2}}^\dagger \of{ -\imJacV^1 \nu -\lambda \error +\featSetDVdot},
\end{equation}
so that
\begin{equation}
  \dot \error = -\lambda \error + \Delta \error,
\end{equation}
where $\Delta \error$ is mismatch between the true solution and the
computed pseudo-inverse solution. If the problem is realizable, then
$\Delta \error$ will vanish and the robot will achieve the target pose.
If $\Delta \error$ does not vanish, then there will be an error (usually
some fixed point $\error_{ss} \neq 0$). It is common for the robot's
forward velocity to be set to a reasonable constant $\nu = \bar \nu$ in
the angular control solution \eqref{eq:IBVSw}. This law drives the
camera frame to the target pose (relative to $\mc W$).

%In the time-varying, trajectory tracking case we assume that a trajectory
%reference $\mcframe{\camF}{W}{C}(t)$ exists along with a control signal
%$u^*(t)$ satisfying \eqref{eq:camDE}. It would typically be derived from
%a robot trajectory reference $\mcframe{\roboF}{W}{R}(t)$ and control signal
%$u^*(t)$ satisfying \eqref{eq:roboDE}. Using those time-varying
%functions, the equations in \eqref{eq:camDE} are solved to obtain the
%image coordinate trajectories. Written in short-hand to expose only the
%main variables, they are:
%\begin{equation} 
%\begin{split}
%  \dot \featureSetD & = \imJac \circ \mcframe{h}{C}{W}(t)(\pointSet^{\mc W}) \cdot
%    \zeta_{u^*(t)}, \ \text{with} \\
%    \featureSetD(0) & = \camProj \circ \mcframe{h}{C}{W}(0)(\pointSet^{\mc W}).
%\end{split}
%\end{equation}
Since the desired feature set is time varying from $\featureSetD(t)$ in equation \eqref{eq:featDE}:
\begin{eqnarray}
\featSetDVdot=\imJacV^1(\pointSetV^{\mc C^*}(t),\featSetDV(t)) \nu^* +\imJacV^2(\pointSetV^{\mc C^*}(t),\featSetDV(t)) \omega^*.
\end{eqnarray} 
The vectorized steering equations \eqref{eq:vStEq} lead to
\begin{multline} \label{eq:IBVStrajTrack}
  \omega = {\of{\imJacV^2(\pointSetV^{\mc C},\featSetV)}}^\dagger
    \bigg( \imJacV^1(\pointSetV^{\mc C^*}(t),\featSetDV(t)) \nu^* 
          -\imJacV^1(\pointSetV^{\mc C},\featSetV) \nu
    \\
      + \imJacV^2(\pointSetV^{\mc C^*}(t),\featSetDV(t)) \omega^* 
      - \lambda \error \bigg).
\end{multline}
They consist of feedforward terms derived from the desired trajectory and
feedback terms to drive the error to zero. The feedforward terms should cancel
out the $\dot \featureSetD$ term in \eqref{eq:ErrorSetDE}, or
equivalently the now non-vanishing $\featSetDVdot$ term in 
\eqref{eq:errorDE}. 
When traveling along the feature trajectory $\featureSetD(t)$, the
angular velocity $\omega$ is computed from \eqref{eq:IBVStrajTrack},
where starred terms and $\nu$ are known quantities.  
To the best of our
knowledge, no general IBVS tracking equations have been derived that combine
feed-forward and feedback control elements.

%It is possible to perform trajectory servoing without VI-SLAM, but then 
%there needs to be a strong feature tracking module, 
%otherwise feature impoverishment and other problems may occur.
%Since visual servoing focuses on the control $u$, exposing its actual
%structure from \eqref{eq:camDE}, \eqref{eq:camPtDot} and
%\eqref{eq:imJac}, leads to
%\begin{equation} \label{eq:camJacu}
%\begin{split}
%  \dot \camPt 
%     = \imJac(q^{\mc C}) 
%      \cdot \Ad^{-1}_{\mcframe{h}{R}{C}} \cdot 
%      \begin{bmatrix} 1 & 0 \\ 0 & 0 \\ 0 & 1 \end{bmatrix}
%      \begin{bmatrix} \nu \\ \omega \end{bmatrix} 
%     = \imJac_u(q^{\mc C}; \mcframe{h}{R}{C}) 
%      \begin{bmatrix} \nu \\ \omega \end{bmatrix}
%\end{split}
%\end{equation}
%where $L_u$ absorbs the linear operations (the Adjoint and matrix product).
%IBVS then relates necessary control effort to corrective maneuvering that
%drives projected points in the image to target coordinates, under the
%assumption that the geometry of the points permits simultaneous
%projection to their targeted coordinates.
%
%Define $\featureSet = \set{\camPt_i}_{1}^{\numFeat} \subset \Real^2$ 
%as a set of image points in the current camera image, sourced from the set  
%$\pointSet = \set{q_i^{\mc W}}_{1}^{\numFeat} \subset \Real^3$ 
%of points in the world frame.  Suppose that the robot should attain a
%future pose given by $\roboF^*$, for which the points in $\pointSet$
%will project to the image coordinates $\featureSetD = \camProj \circ
%(\roboF^* \mcframe{\camF}{R}{C})^{-1}(\pointSet)$. For simplicity, ignore
%field of view issues and occlusions between points. Their effect would be
%such that only a subset of the points in $\pointSet$ would permit use
%for visual servoing. Assume that we are already working with
%this feasible set whereby the indexed elements in $\featureSet$
%correspond exactly to their counterpart in $\featureSetD$ with the same
%index, i.e., the sets are {\em in correspondence}.
%
%Define the error to be $\errorSet = \featureSet - \featureSetD$ where
%elements with matched indices are subtracted. The error dynamics of the
%points are:
%\begin{equation} \label{eq:ErrorSetDE}
%  \errorSet = \dot \featureSet - \dot \featureSetD = 
%    \imJac_u(\mcframe{\camF}{C}{W}(\pointSet), \featureSet; \mcframe{h}{R}{C}) \cdot u - \dot \featureSetD
%\end{equation}
%where we apply the same argument adjustment as in \eqref{eq:imJac} so
%that dependence is on image features then point coordinates as needed.
%Further, functions or operations applied to indexed sets will return an
%indexed set whose elements correspond to the input elements from the
%input indexed set. Since the desired image coordinates $\featureSetD$
%are with respect to a static goal pose, $\dot \featureSetD = 0$.
%Define $\error$, $\featSetV$, $\featSetDV$, and $\imJacV$ to be the
%vectorized versions
%of $\errorSet$, $\featureSet$, $\featureSetD$ and $\imJac$. Then,
%\begin{equation} \label{eq:errorDE}
%  \dot \error =
%  \imJacV(\mcframe{\camF}{C}{W}(\pointSetV),\featSetV;\mcframe{h}{R}{C}) \cdot u
%    - \featSetDVdot
%  =
%  \imJacV(\mcframe{\camF}{C}{W}(\pointSetV),\featSetV;\mcframe{h}{R}{C}) \cdot u 
%\end{equation}
%is an overdetermined set of equations for $u$ when $\numFeat > 2$.
%Removing the functional dependence and breaking apart the different
%control contributions, the objective is to satisfy,
%\begin{equation} \label{eq:IBVSw}
%  \dot \error = \imJacV \cdot u = \imJacV^1 \nu + \imJacV^2 \omega 
%              = -\lambda \error.
%\end{equation}
%A solution is to define,
%\begin{equation}
%  \omega = {\of{\imJacV^2}}^\dagger \of{ -\imJacV^1 \nu -\lambda \error},
%\end{equation}
%so that
%\begin{equation}
%  \dot \error = -\lambda \error + \Delta \error,
%\end{equation}
%where $\Delta \error$ is mismatch between the true solution and the
%computed pseudo-inverse solution. If the problem is realizable, then
%$\Delta \error$ will vanish and the robot will achieve the target pose.
%If $\Delta \error$ does not vanish, then there will be an error (usually
%some fixed point $\error_{ss} \neq 0$). It is common for the robot's
%forward velocity to be set to a reasonable constant $\nu = \bar \nu$ in
%the angular control solution \eqref{eq:IBVSw}. This law drives the
%camera frame to the target pose (relative to $\mc W$).
%
%In the time-varying, trajectory tracking case we assume that a trajectory
%reference $\mcframe{\camF}{W}{C}(t)$ exists along with a control signal
%$u^*(t)$ satisfying \eqref{eq:camDE}. It would typically be derived from
%a robot trajectory reference $\mcframe{\roboF}{W}{R}(t)$ and control signal
%$u^*(t)$ satisfying \eqref{eq:roboDE}. Using those time-varying
%functions, the equations in \eqref{eq:camDE} are solved to obtain the
%image coordinate trajectories. Written in short-hand to expose only the
%main variables, they are:
%\begin{equation} \label{eq:featDE}
%\begin{split}
%  \dot \featureSetD & = \imJac \circ \mcframe{h}{C}{W}(t)(\pointSet^{\mc W}) \cdot
%    \zeta_{u^*(t)}, \ \text{with} \\
%    \featureSetD(0) & = \camProj \circ \mcframe{h}{C}{W}(0)(\pointSet^{\mc W}).
%\end{split}
%\end{equation}
%Since the desired feature set is time varying, $\featureSetD(t)$, the
%vectorized steering equations lead to
%\begin{multline} \label{eq:IBVStrajTrack}
%  \omega = {\of{\imJacV^2(\pointSetV^{\mc C},\featSetV)}}^\dagger
%    \bigg( \imJacV^1(\pointSetV^{\mc C^*}(t),\featSetDV(t)) \nu^* 
%          -\imJacV^1(\pointSetV^{\mc C},\featSetV) \nu
%    \\
%      + \imJacV^2(\pointSetV^{\mc C^*}(t),\featSetDV(t)) \omega^* 
%      - \lambda \error \bigg).
%\end{multline}
%They consist of feedfoward terms derived from the desired trajectory and
%feedback terms to drive the error to zero. The feedforward terms should cancel
%out the $\dot \featureSetD$ term in \eqref{eq:ErrorSetDE}, or
%equivalently the now non-vanishing $\featSetDVdot$ term in 
%\eqref{eq:errorDE}. 
%
%%\color{red}
%%WHAT PURPOSE???
%%\textbf{Note 1:} it may be useful to compute multiple desired feature
%%sets for multiple consecutive poses, and generate a better current
%%control through some cost functions. Is it possible to form an
%%optimization formula to solve this? Also it looks similar to receding
%%horizon. This could be a different research topic.
%%
%%\textbf{Note 2:} also need to check if the robot reaches the desired pose
%%$\pose_d$. It may be sufficient to check if my current pose is close to
%%the desired in the local frame.
%%\color{black}
%
%\subsection{Trajectory Servoing}
%
%%IBVS presented in the last section is a useful tool to achieve this task.
%
%
%The IBVS equations presented in the previous section are for tracking
%a specified camera trajectory using image feature point measurements
%with known static positions in the world.  The prerequisites needed to
%solve \eqref{eq:featDE} and implement \eqref{eq:IBVStrajTrack} are the
%major challenges regarding the use of visual servoing to navigate
%unknown environments.  
%They are all possible to meet based on the information and modules
%available within the software stack of an autonomous mobile robot.  
%This section describes the basic {\em trajectory servoing}
%implementation and describes how to build a solution that satisfies the
%prerequisites. It focuses on short-term navigation where sufficient
%image features remain within the field of view for the entire trajectory.
%
%%Prerequisites:
%%1. working with feasible set. Indexed elements are in correspondence.
%%2. we have a path defined forward in time, starting at the current
%%robot pose or sufficiently nearby.
%%3. trajectory is forward simulated under control policy to obtain the
%%target trajectory with control terms (for feedforward and feedback
%%control). This gives the robot reference and control (after (11). The
%%robot reference is then mapped to the camera reference.
%%4. we can maintain association of features over time.
%%5. Around  (11), "if the problem is realizable." It is realizable based
%%on forward integration of earlier equations.
%%6. (12) and (13) can be implemented.
%
%The trajectory servoing needs condense down to the following:
%(1) A set of points with known (relative) positions;
%(2) A given trajectory and control signal for the robot starting at
%the robot's current pose (or nearby); and
%(3) The ability to index and associate them across future image
%  measurements when tracking the trajectory.
%The autonomy modules that contribute this information are the
%navigation and SLAM stacks. A typical hierarchical navigation stack
%will generate a local trajectory to follow in realization of a
%long-term objective. An indirect, feature-based SLAM stack will keep
%track of points in the local environment and link them to previously
%observed visual features while also estimating their actual position
%relative to the robot.  
%
%\subsubsection{The trajectory and control signals}
%%For the intents of this section, we will 
%Assume that a specific short-duration path has been established as the
%one to follow, and has been converted into a path relative to the
%robot's local frame. It either contains the current robot pose in it,
%or has a nearby pose.
%Contemporary navigation stacks have a means to synthesize both a time
%varying trajectory and an associated control signal from the paths.
%Here, we apply a standard trajectory tracking controller to generate
%$\roboBV^*(t)$ and $\mcframe{\roboF}{W,*}{R}(t)$ by forward simulating
%\eqref{eq:roboDE}
%(note that $\roboBV^*$ contains the linear velocity $\nu^*$ and angular
%velocity $\omega^*$).  Some navigation stacks use optimal control
%synthesis to build the trajectory.  Either way, the generated
%trajectory is achievable by the robot, which means that the forward
%integrated terms in \eqref{eq:featDE} will lead to a realizable visual
%servoing problem where $\nu^*$, $\omega^*$, and $\featSetDV(t)$ are
%consistent with each other. The equations will require converting the
%robot trajectory to a camera trajectory
%$\mcframe{\camF}{W,*}{C}(t)$ using $\Ad^{-1}_{\mcframe{h}{R}{C}}$. 
%
%\subsubsection{The features and feature paths}
%The SLAM module provides a pool of visible features with known relative
%position for the current stereo frame, plus a means to assess future
%visibility if desired. Taking this pool to define the 
%feature set $\featureSetD(0)$ gives the final piece of information
%needed to forward integrate \eqref{eq:featDE} and generate feature 
%trajectories $\featureSetD(t)$ in the left camera
%frame. This process acts like a short-term teach and repeat 
%feature trajectory planner but is sim and repeat. 
%
%A less involved module could be used besides a fully realized SLAM
%system, however doing so would require creating many of the fundamental
%building blocks of an indirect, feature-based SLAM system. 
%%Components needed include feature detection, feature matching, and map
%%point estimation.  Map point estimation could be removed, but at the
%%consequence of introduction error in the map point depth estimation
%%from individual stereo measurement. 
%Given the availability of strong performing open-source, real-time SLAM
%methods, there is little need to create a custom module.
%
%%It is possible to perform trajectory servoing without VI-SLAM, but then 
%%there needs to be a strong feature tracking module, 
%%otherwise feature impoverishment and other problems may occur.
%
%\subsubsection{Trajectory Servoing Control}
%When traveling along the feature trajectory $\featureSetD(t)$, the
%angular velocity $\omega$ is computed from \eqref{eq:IBVStrajTrack},
%where starred terms and $\nu$ are known quantities.
%
%%The derivation of the IBVS feedback law in the time-varying case requires a set of properties or constraints to hold. They may appear to be limited, however they are all possible to achieve based on the local navigation task and the existing data avilable from the navigation system. This subsection describs from where the information is obtained and how it is used to synthesize a feasible problem. Basically the local planner provides trajectories with control signals. The SLAM system provides the world points in local coordinates (or global, whatever seems best; local I would say but who knows). These are combined to generate the forward path of the feature points.
%%
%%Explain how the setup differs from published works. Basically they did not consider the type of fully fledged navigation system we have. Removing the local path or the SLAM mapping ends up undermining the ability to perform the task. It is possible without SLAM, but then there needs to be a strong feature tracking module, otherwise there will be feature impoverishment and other problems. Using purely IBVS and final pose causes weird motions. The smaller the different between the current feature coordinates and the target ones, the better posed the problem (less chances of weird behavior, better tracking, etc.). This has been known for 15 years (earlier papers). Basically, cover the rationale behind the solution. It is not an accident that the current pipeline is the one we converged to. Think back to what you all explored this year and how it evolved.
%
%%The image feature sets $\featureSet$, $\featureSetD(0)$ or 
%%their sources $\pointSet^{\mc W}$ are obtained from a stereo VI-SLAM system,
%%which can increasing the stability of trajectory servoing 
%%through these well-tracked features and triangulated depth information from 
%%the stereo camera.
%
%%\toedit{
%%The prior works ... has introduced how to track a trajectory using SLAM
%%pose and evaluate the values that will affect the tracking error.
%% Therefore, it is necessary to design a system that does not
%%explicitly depend on the localization. }







==> arxiv_submission/shortExp.tex <==
%\newcommand{\sym}{\raisebox{\depth}{$\diamondsuit$}}
\subsection{Experiments and Results}\label{sec:shortDist_exp}

This section runs several short distance trajectory servoing
experiments to evaluate the accuracy of the image-based feedback
strategy supplemented by stereo SLAM. The hypothesis is that mapping
trajectory tracking to image-space will improve short term trajectory
tracking by removing the impact of SLAM estimation drift from the
feedback loop. 

\subsubsection{Experimental Setup}
For quantifiable and reproducible outcomes, the ROS/Gazebo SLAM
evaluation environment from \cite{zhao2020closednav} is used for
the tests.  Fig. \ref{fig:tsrb_env} shows a top down view of the world
plus a robot view. The simulated robot is a Turtlebot.  
It is tasked to follow a specific short-distance trajectory.
A total of five paths were designed, loosely based on Dubins paths. They
are denoted as straight (S), weak turn (WT), straight+turn (ST),
turn+straight (TS), turn+turn (TT), and are depicted in Fig.
\ref{fig:short_paths}. Average length of all trajectories are $\sim$4m.
Longer paths would consist of multiple short segment reflecting
variations on this path set.  They are designed to ensure that
sufficient feature points visible in the first frame remain visible
along the entirety of the path. Five trials per trajectory are run.  The
desired and actual robot poses are recorded for performance scoring.
Performance metrics computed are average translation error (ATE).

\subsubsection{SLAM Stack}
Part of the robot's software stack includes the Good Feature (GF) ORB-SLAM
system \cite{8964284} for estimating camera poses. It is configured to
work with a stereo camera and integrated into a loosely coupled,
visual-inertial (VI) system \cite{zhao2020closednav,20.500.11850/52698} based on a 
multi-rate filter to form a VI-SLAM system. The trajectory servoing system will interface with
the GF-ORB-SLAM system to have access to tracked features for IBVS.


%Three different trajectory tracking methods are investigated. 
%1) Pose-based trajectory tracking with ground truth robot poses in the
%simulation.  This trajectory tracking method includes a feedback term
%to measure the difference between current robot pose and desired
%trajectory pose, and a feedforward term to consider the desired
%velocities.  In the Gazebo simulation, the ground truth robot pose is
%obtained to apply in this trajectory tracking. 
%These poses are used as a baseline for the comparison, and impossible
%in reality.  2) Same trajectory tracking method with estimated robot
%poses from VI-SLAM. 


\begin{table*}[t]
  \vspace*{0.06in}
  \addtolength{\tabcolsep}{-2.5pt}
  \centering
  \begin{minipage}[t]{0.28\textwidth}
    \centering
    \caption{\textrm{Trajectory Tracking ATE (cm)}%
    \label{tb:shortTrajBench}}
    \begin{tabular}{|c||cccc|}
    \hline 
    \textbf{Seq.} & PO & SLAM & TS & VS+ \\ 
    \hline 
%       &       &       & SLAM  & $\neg$SLAM \\
    S  & 2.27  & 3.67  & 0.76  & x \\ 
    WT & 1.62  & 3.62  & 0.76  & x \\ 
    ST & 2.50  & 2.96  & 1.06  & x \\ 
    TS & 1.58  & 3.24  & 1.33  & x \\ 
    TT & 2.35  & 3.50  & 1.04  & x \\ 
    \hline 
    \textbf{Avg. ATE} & 2.06 & 3.40 & \textbf{\em 0.99} & x \\ 
    %\textbf{Std. ATE} & 0.0000 & 0.0000 & 0.0000 \\
%    & \textcolor{white}{$v,\omega$} & & & \\
    \hline 
    \end{tabular}
  \end{minipage}
%  \hspace*{1pt}
  \begin{minipage}[t]{0.2\textwidth}
    \centering
    \caption{\textrm{Terminal Error (cm)}%
    \label{tb:shortTrajTE}}
    \begin{tabular}{|c||ccc|}
    \hline 
    \textbf{Seq.} & PO & SLAM & TS \\ 
    \hline 
%      & \textcolor{white}{$v,\omega$} & & \\
    S  & 2.47  & 5.44  & 1.29  \\ 
    WT & 1.83  & 5.93  & 1.30  \\ 
    ST & 2.85  & 1.50  & 2.99  \\ 
    TS & 1.85  & 1.76  & 2.04  \\ 
    TT & 2.34  & 3.07  & 2.27  \\ 
    \hline 
    \textbf{Avg.} & 2.27 & 3.54 & \textbf{\em 1.98} \\ 
    %\textbf{Std. ATE} & 0.0000 & 0.0000 & 0.0000 \\
%    & \textcolor{white}{$v,\omega$} & \\
    \hline 
    \end{tabular}
  \end{minipage}
%  \hspace*{-7pt}
  \begin{minipage}[t]{0.18\textwidth}
    \centering
    \caption{\textrm{Estimation ATE (cm)}%
    \label{tb:shortEst}}
    \begin{tabular}{|c||cc|}
    \hline 
    \textbf{Seq.} & SLAM & TS \\ 
    \hline 
%      & \textcolor{white}{$v,\omega$} & \\
    S  & 1.16 & 1.41 \\ 
    WT & 1.63 & 1.66 \\ 
    ST & 2.48 & 3.00 \\ 
    TS & 4.22 & 3.91 \\ 
    TT & 3.75 & 3.36 \\
    \hline 
    \textbf{Avg.} & 3.02 & \textbf{\em 2.67} \\ 
    %\textbf{Std. ATE} & 0.0000 & 0.0000 \\
%    & \textcolor{white}{$v,\omega$} & \\
    \hline 
    \end{tabular}
  \end{minipage}
%  \hspace*{-7pt}
  \begin{minipage}[t]{0.3\textwidth}
    \centering
    \caption{\textrm{Control Effort}
    \label{tb:shortCost}}
    \begin{tabular}{|c||cccccc|}
    \hline 
    \textbf{Seq.} & \multicolumn{2}{c}{PO} & \multicolumn{2}{c}{SLAM} & \multicolumn{2}{c|}{TS}\\ 
    \hline 
    • & $\nu$ & $\omega$ & $\nu$ & $\omega$ & $\nu$ & $\omega$\\ 
    S  & 7.88 & 0.20 & 7.10 & 0.19 & 5.86 & 1.17 \\ 
    WT & 8.14 & 0.55 & 7.35 & 0.48 & 6.16 & 1.84 \\ 
    ST & 7.58 & 4.73 & 6.70 & 3.47 & 5.67 & 3.38 \\ 
    TS & 8.18 & 4.92 & 7.33 & 4.27 & 6.19 & 4.46 \\ 
    TT & 8.47 & 4.82 & 7.72 & 4.24 & 6.46 & 4.75 \\ 
    \hline 
    \textbf{Avg.} & 8.05 & 3.04 & 7.24 & \textbf{2.53} & \textbf{\em 6.07} & \em 3.12 \\ 
    • & \multicolumn{2}{c}{11.09} & \multicolumn{2}{c}{9.77} & \multicolumn{2}{c|}{\textbf{\em 9.19}} \\
    \hline 
    \end{tabular} 
  \end{minipage}
  \addtolength{\tabcolsep}{2pt}
  \vspace*{-0.15in}
\end{table*}

%\begin{table}[h]
%  \centering
%  \begin{minipage}[t]{0.5\textwidth}
%    \centering
%    \caption{\textrm{Control Effort}
%    \label{tb:shortCost}}
%    \begin{tabular}{|c||cccccc|}
%    \hline 
%    \textbf{Seq.} & \multicolumn{2}{c}{PO} & \multicolumn{2}{c}{SLAM} & \multicolumn{2}{c|}{TS}\\ 
%    \hline 
%    • & $\nu$ & $\omega$ & $\nu$ & $\omega$ & $\nu$ & $\omega$\\ 
%    S  & 7.88 & 0.20 & 7.10 & 0.19 & 5.86 & 1.17 \\ 
%    WT & 8.14 & 0.55 & 7.35 & 0.48 & 6.16 & 1.84 \\ 
%    ST & 7.58 & 4.73 & 6.70 & 3.47 & 5.67 & 3.38 \\ 
%    TS & 8.18 & 4.92 & 7.33 & 4.27 & 6.19 & 4.46 \\ 
%    TT & 8.47 & 4.82 & 7.72 & 4.24 & 6.46 & 4.75 \\ 
%    \hline 
%    \textbf{Avg.} & 8.05 & 3.04 & 7.24 & \textbf{2.53} & \textbf{\em 6.07} & \em 3.12 \\ 
%    • & \multicolumn{2}{c}{11.09} & \multicolumn{2}{c}{9.77} & \multicolumn{2}{c|}{\textbf{\em 9.19}} \\
%    \hline 
%    \end{tabular} 
%  \end{minipage}
%\end{table}

\begin{figure}[t]
  \vspace*{0.06in}
  \centering
  {\includegraphics[height=1.25in]{figs/ICRA2021Figs/ShortFigs/GazeboEnv/tsrb_env.png}}
  {\includegraphics[height=1.25in]{figs/ICRA2021Figs/ShortFigs/features/feature3.png}}
  \vspace*{-0.1in}
  \caption{Gazebo environment top view and robot view with SLAM features.\label{fig:tsrb_env}}
%\end{figure}
%\begin{figure}[t]
  %\vspace*{-0.1in}
  \centering
  \begin{tikzpicture}[inner sep=0pt, outer sep=0pt]
  \node (S) at (0in,0in) 
    {\includegraphics[width=21.8pt]{figs/ICRA2021Figs/ShortFigs/shortTrajs/S.png}};
  \node[anchor=south west,xshift=10pt] (WT) at (S.south east)
    {\includegraphics[width=26.9pt]{figs/ICRA2021Figs/ShortFigs/shortTrajs/T.png}};
  \node[anchor=south west,xshift=10pt] (ST) at (WT.south east)
    {\includegraphics[width=39.2pt,clip=true,trim=0in 0in 0in 1.0in]{figs/ICRA2021Figs/ShortFigs/shortTrajs/ST.png}};
  \node[anchor=south west,xshift=10pt] (TS) at (ST.south east)
    {\includegraphics[width=26.9pt,clip=true,trim=0in 0in 0in 1.0in]{figs/ICRA2021Figs/ShortFigs/shortTrajs/TS.png}};
  \node[anchor=south west,xshift=10pt] (TT) at (TS.south east)
    {\includegraphics[width=24.4pt,clip=true,trim=0in 0in 0in 1.0in]{figs/ICRA2021Figs/ShortFigs/shortTrajs/TT.png}};

  \node[anchor=north] at (S.south) {\footnotesize S};
  \node[anchor=north] at (WT.south) {\footnotesize WT};
  \node[anchor=north] at (ST.south) {\footnotesize ST};
  \node[anchor=north] at (TS.south) {\footnotesize TS};
  \node[anchor=north] at (TT.south) {\footnotesize TT};
  \end{tikzpicture}
  \vspace*{-0.5em}
  \caption{Short-distance template trajectories.  \label{fig:short_paths}}
  \vspace*{-1em}
\end{figure}

\subsubsection{Methods Tested}
In addition to the trajectory servoing algorithm, several baseline
methods are implemented. The first is a pose feedback strategy using
{\em perfect odometry} (PO) as obtained from the actual robot pose in
the Gazebo simulator. The second replaced PO with the SLAM estimated pose, 
which are delayed and have uncertainty. The third is a
trajectory servoing method without the V-SLAM system, which would be
a naive implementation of visual servoing based on \eqref{eq:IBVStrajTrack}.
It is called VS+ to differentiate from trajectory servoing, and uses a 
frame-by-frame stereo feature tracking system \cite{stvo_repo}. 
Pose-based control \cite{zhao2020closednav} uses a geometric
trajectory tracking controller with feedforward $[\nu^{*},\omega^{*}]^T$
and feedback
\begin{equation} \label{eq:poseController}
\begin{split}
\nu_{cmd} & = k_{x}*\widetilde{x} + \nu^{*} \\
w_{cmd} &= k_{\theta}*\widetilde{\theta} + k_{y}*\widetilde{y} + \omega^{*} \\
\end{split}
\end{equation}
where,
\begin{equation} \label{eq:GErr}
  [\widetilde{x},\widetilde{y},
  \raisebox{-1.5pt}{$\widetilde{\theta}$}\makebox[2\width]{$]$}^T \simeq
  \widetilde{g} = \inverse{\roboF} \roboF^* = 
    \inverse{\of{\mcframe{\roboF}{W}{R}}}(t) 
    \of{\mcframe{\roboF}{{W},*}{R}}(t).
\end{equation}
The controller gains have been empirically tuned to give good
performance for the perfect odometry case, and have been extensively used 
in prior work \cite{zhao2020closednav,Smith2017,Smith2020}.

\subsubsection{Results and Analysis}
Tables \ref{tb:shortTrajBench} to \ref{tb:shortCost} quantify the
outcomes of all methods tested.  Fig. \ref{fig:shortTrajBench} consists
of boxplots of the trajectory tracking error for the different template
trajectories and methods (minus VS+). 
The first outcome to note is that VS+ fails for all paths.  The average
length of successful servoing is 0.4m ($\sim$10\% of the path length).
Inconsistent data association rapidly degrades the feature pool and
prevents consistent use of feature for servoing feedback.  Without the
feature map in V-SLAM, a reappeared feature will be treated as a new
feature and assigned with a different index, which easily violates the
{\em correspondence} rule from \S\ref{FeatPaths}.  As noted there, any
effort to improve this would increasingly approach the computations
found in a V-SLAM method.  Maintaining stable feature tracking through
V-SLAM is critical to trajectory servoing.

Comparing SLAM and TS, the Table values show lower errors across the
board, and lower control cost.  Trajectory tracking error is lower by
71\% and terminal error is lower by 44\%. Interestingly, the pose
estimation error is only reduced by around 12\%, which indicates weak
improvement in pose estimation from the better tracking via TS. This is
most likely a result of the SLAM pose predictions being decoupled from
the control system, leading to uninformed motion priors.  ORB-SLAM uses
a motion prior based on its own internal estimates.  Tightly coupling
the two parts may improve the SLAM system, but may also introduce new
sensitivities. The TS approach reduces control effort by 19\%.

Comparing PO with TS shows better performance by TS, which was not
expected. This might suggest some additional tuning would be necessary.
However, usually there is trade-off between tracking error and control
cost. Attempts to improve tracking usually increase the control cost,
and vice-versa. Based on the values of the Tables, it is not clear that
better would be possible. Tests later in this manuscript will show that
the benefit does not persist for longer paths, thus the improvement for
short trajectories is of limited use.
The finding here is that implementing a purely image-based approach to
trajectory tracking through unknown environments is possible, and can
work well over short segments in the absence of global positioning
information.  

%The trajectory servoing system has the lowest error of the methods,
%which demonstrates that the hypothesis was met.  Interestingly, it also
%outperforms the case of feedback using the true pose.  

%The same statistics are given in Table \ref{tb:shortTrajBench} and show
%TS outperforming PO and SLAM by 52\% and 71\%.  Similarly, from
%\ref{tb:shortTrajTE}, the terminal error of TS is also reduced by 13\%
%and 44\%.
%Lastly, from Table \ref{tb:shortCost}, the control effort of TS in $\nu$
%is the lowest, with PO and SLAM overactuating by 33\% and 19\%.
%It also suggests that there may be an increase
%in steering control effort for short term trajectory servoing.
%The overall control effort of TS reduces 17\% and 6\% from PO and SLAM. 
%Comparing to SLAM, PO sacrifices control effort to obtain a lower tracking error. But trajectory servoing can achieve better performance with even 
%lower control effort.

%The robot trajectory and pose estimation based on SLAM are drifted. 
%In addition, the trajectories of pose-based controllers \cite{9197003} will exceed the desired trajectory, which shows their inaccuracy to control the linear velocities compared with the trajectory servoing with feedforward. 
%This inaccuracy may be resolved by fine-tuning the multiple control gains, 
%but it is much easier for trajectory servoing to choose one simple $\lambda$ in 
%Equation \eqref{eq:IBVStrajTrack}.  Furthermore, the pose estimation is
%not smooth that could be caused by sensor noise and sensor fusion
%process.  This facts will contribute to the high error range of the
%pose-based trajectory tracking with SLAM pose.

\begin{figure}[t]
  \centering
%  \fbox{\includegraphics[width=3in,clip=true,trim=4in 3in 0in 0.25in]{figs/shortbox_update.png}}
	{\includegraphics[width=2.5in,clip=true,trim=0in 0in 0in 0in]{figs/shortbox_fixed.png}}
  \vspace*{-0.5em}
  \caption{Short-distance trajectory benchmarking results%
  \label{fig:shortTrajBench}}
  \vspace*{-1em}
\end{figure}



==> filter_exp.tex <==
\begin{table*}[t]
  \vspace*{0.06in}
  \addtolength{\tabcolsep}{-2.5pt}
  \centering
  \begin{minipage}[t]{0.45\textwidth}
    \centering
    \caption{\textrm{Random Blue Policy Evaluation Metrics}%
    \label{tb:randomBlueFilter}}
    \begin{tabular}{|c||ccccc|}
    \hline 
    \textbf{Filt.} & RT & LL & ADE & CTP & DESV (1-$\sigma$)\\ 
    \hline 
    LSTM  & 8.93e-4  & 1.74  & 1.38e-1  & 4.27e-1 & 2.99e-1\\ 
    GNN & 7.14e-3  & 2.93  & 7.91e-2  & 5.12e-1 & 3.26e-1\\ 
    VRNN & 8.85e-3  & 4.70  & 4.59e-2  & 9.01e-1 & 2.77e-1\\ 
    VRNN-GNN & 1.51e-2  & 3.61  & 6.13e-2  & 7.14e-1 & 4.12e-1\\ 
    Kalman & N/A  & N/A  & 6.29e-2  & N/A & N/A\\ 
    Prior-Only & 5.01e-4  & 5.30  & 1.37e-1  & 9.67e-1 & 2.55e-1\\ 
    Combined & 9.17e-4  & 7.25  & 4.19e-2  & 9.71e-1 & 4.89e-1\\
    MLP & 5.02e-4  & 5.73  & 5.74e-2  & 9.63e-1 & 3.06e-1\\
    \hline 
    \end{tabular}
  \end{minipage}
  \begin{minipage}[t]{0.45\textwidth}
    \centering
    \caption{\textrm{Heuristic Blue Policy Evaluation Metrics}%
    \label{tb:heuBlueFilter}}
    \begin{tabular}{|c||ccccc|}
    \hline 
    \textbf{Filt.} & RT & LL & ADE & CTP & DESV (1-$\sigma$)\\ 
    \hline 
    LSTM  & 8.88e-4  & 1.74  & 1.28e-1  & 4.43e-1 & 3.13e-1\\ 
    GNN & 7.56e-3  & 4.74  & 5.23e-2  & 8.11e-1 & 4.26e-1\\ 
    VRNN & 9.11e-3  & 5.13  & 5.46e-2  & 8.67e-1 & 3.81e-1\\ 
    VRNN-GNN & 1.42e-2  & 5.33  & 7.69e-2  & 8.07e-1 & 4.42e-1\\ 
    Kalman  & N/A  & N/A  & 3.40e-2  & N/A & N/A\\
    Prior-Only & 4.93e-4  & 2.71  & 1.79e-1  & 6.92e-1 & 1.84e-1\\ 
    Combined & 9.24e-4  & 7.57  & 3.41e-2  & 9.66e-1 & 5.13e-1\\
    MLP & 4.90e-4  & 6.15  & 4.16e-2  & 8.92e-1 & 3.96e-1\\
    \hline 
    \end{tabular}
  \end{minipage}

  \addtolength{\tabcolsep}{2pt}
  \vspace*{-0.15in}
\end{table*}


%\newcommand{\sym}{\raisebox{\depth}{$\diamondsuit$}}
\subsection{Experiments and Results}\label{sec:filter_exp}

This sections trains several different above mentioned models and compares them with respect to various metrics. The hypothesis is that the MDN based prior-dynamic combined model can improve the accuracy of the filter compared with other common baselines by balancing the importance of the two information sources with learned weights. 

\subsubsection{Experimental Setup}
Here we use the Prisoner Escape environment as \ref{sec:environment} describes. The prisoner is going to reach a hideout while being minimally detected by the searchers with a policy composed of an A* search planner (Fig \ref{fig:astar}) and an evasive behavior maneuver. The A* planner minimizes a cost with a combination of the terrain visibility and distance between start and goal. Intuitively, it remain as hidden as possible while taking the shortest distance to the goal. The prisoner also attempts to change its velocity and escape to the dark forest if detected for a short time and recovers to A* path when gets rid of \SA{} or detected for too long. The upper limit speed of the prisoner, the search parties and the helicopter is 15, 20 and 127 grids/step respectively. 

\begin{figure}[t]\label{fig:astar}
	\centering
	% \includegraphics[width=0.45\textwidth]{figs/environment/path_a_star.png}
 	\includegraphics[width=0.45\textwidth]{figs/environment/path_evasion.png}
	\caption{A* Path Planner from Start to Hideout}
\end{figure}


At the start of the MARL training, each searching agent uses a randomly initialized policy which means very few detections of the prisoner occur. Thus only sparse useful information is available for the training. This is one important reason why we need to append the filter output to the MARL observation as extra information to facilitate its tracking policy training. Additionally, we need to evaluate the filter with the random searching policies of blue agents to match the data distribution at the beginning of MARL. Specifically, we record \notsure{500} rollouts and divide with \notsure{} training samples, \notsure{} validating samples and \notsure{} test samples to evaluate. We also do the same for the heuristic searching policies to see how the filters work in a larger detection rate environment which corresponding to the half-way MARL training. For quantifiable and reproducible outcomes, we use the same random seeds \notsure{,} for the training and testing above respectively.

\subsubsection{Methods Tested}
\color{red}
We compare our proposed filtering model against various filter configurations. [TODO: Why / How did we choose these baselines??] The inputs to the following filtering approaches include the detection history of the adversary, the location and type of all the tracking agents, a flag to indicate which agent(s) detected the adversary, the position and velocity of the adversary if detected, and the locations of the known hideouts.
% For encoders, we test four baselines. 
% (1) LSTM: An LSTM network with a vector holding all agent histories as the input, (2) Graph-LSTM (GNN): A homogeneous GNN where we construct the graph as defined in \ref{sec:graph_input}, and (3 and 4) VRNN and Graph-VRNN: a Variational RNN \cite{chung2015}. We test all these models without any of the additional contrastive losses.

\begin{itemize}
    \item LSTM: We utilize a standard Long-Short Term Memory (LSTM) network \cite{gers2000learning} to learn an embedding from the history of detections $\{d_i\}_{i=1}^{N_d}$, which is then passed to the MDN. 
    \item GNN: We construct a homogeneous, fully connected GNN, where each node represents the tracking agents.  Each node utilizes a history of the individual agent's observations passed through an LSTM. We then perform graph convolutions and use the average embedding from the graph to feed into the MDN. 
    \item VRNN: The Variational Recurrent Neural Network (VRNN) \cite{chung2015recurrent} consists of a Variational Autoencoder (VAE) at every timestep to model the dependencies between latent random variables across subsequent timesteps. The final hidden state from the VRNN is passed to the MDN.
    % The VRNN utilizes a conditional prior distribution $z_t$ and  approximate posterior that are both dependent on the prior hidden state $h_{t-1}$.
    \item VRNN-GNN: The VRNN-GNN uses graph convolutions similar to the GNN but uses the VRNN instead of LSTMs as the pre-processing recurrent encoding network for each of the agent nodes in the graph.
    \item @Zixuan are we describing MLP, Kalman, also here ..?  \\
\end{itemize}
\color{black}
\subsubsection{Evaluation Metrics}
% \Manishawrite{WRITE: Manisha, please write several sentences and equations to introduce the metrics LL, ADE, CTP, DESV}
For our evaluation, we assume that we have access to the ground truth (GT) locations of the adversary. For models that output a mixture of Gaussians, we calculate the following metrics with respect to each of the predicted gaussian mixture components and weigh them by their respective mixing coefficients.
\begin{itemize}
    \item \textbf{Log-Likelihood (LL):} The average LL of the GT adversary location with respect to the predicted output distribution.
    \item \textbf{Average Displacement Error (ADE):} The mean Euclidean distance between the GT and the predicted adversary location.
    \item \textbf{Confidence Threshold (CTP):} The fraction of time steps in each rollout for which the model predicts that the opponent is within a distance $\delta=0.05$ from the GT location with probability greater than some threshold (say $p >=0.5$).
    \item \textbf{Delta Empirical Sigma Value (DESV(1-$\sigma$)):} The difference in the fraction of timesteps in which the GT positions fall within the $1-\sigma$ level set of the predicted distribution and the fraction from a unit-variance Gaussian distribution. Here we consider the unit variance Gaussian as the ideal gaussian. $\Delta ESV$ is a metric used for identifying over- or under-confidence as $\Delta ESV = \sigma_{\text{pred}} - \sigma_{\text{ideal}}$, with  $\sigma_{\text{ideal}} \approxeq 0.39$ \cite{}. $\Delta ESV < 0$ indicates high-confidence (or $\sigma^2 < 1$), and $\Delta ESV > 0$ indicates low-confidence (or $\sigma^2 > 1$). DESV(1-$\sigma$) has been used in prior work in trajectory forecasting \cite{ivanovic2022propagating}.
    \toedit{@Zixuan, for the DESV metrics, please subtract your values from 0.39 and then report in the table}
\end{itemize}

\subsubsection{Results and Analysis}
We show the average results tested on the evaluation dataset for each filter with respect to the metrics above (Tables \ref{tb:randomBlueFilter} and \ref{tb:heuBlueFilter}) and all the samples in Figure \ref{fig:randomBlue} \ref{fig:heuBlue}. Specifically, we collect all the observation samples in the evaluation set as the input to each model and then calculate the metrics using the filter output and ground truth from the samples.

We can categorize the filters into two groups. \Manishawrite{Group I consists of commonly used recurrent neural network approaches with and without graph convolutions, namely --}LSTM, GNN, VRNN, and VRNN-GNN, to which our proposed filtering model is compared. Group II consists of our proposed combined model and its sub-components - the Kalman, Prior-Only models. We consider it as an ablation study to show how much our combined model improves from its components.

\vspace{3pt}

\noindent \textbf{Random Search Policy Analysis: } We simulate the sparse detection situation by setting each searching agent to take random actions at each timestep. We find that the log-likelihood and the average distance error of the combined model are better than the prior-only model by 27.71\% and 134.88\%, respectively, which is expected since the combined one contains the detection information. We find that Group 1 is worse than the prior-only model by 69.09\%, 47.96\%, 16.52\%, and 35.88\% with respect to the LL. However, the ADE of the prior-only model is larger than the baselines. It shows that the RNN and GNN-based methods with full observation sequence (both environment variables and detection information) have poorer performance than the prior-only model, which only takes in the environment variables. However, the prior-only model has a larger ADE since it could never infer the probability of which path it is traveling from the detection\ref{}. This corresponds our hypothesis that it is difficult to balance the prior knowledge which indicates the path preference and the detection in a unified network and inspires the motivation to design the combined network which process the two source of information in two passes and then integrate with a learnable weight. \Manishawrite{Further, we find that our combined model has the highest Confidence Threshold, and our prior model and the MLP also perform better than the Group I models. In terms of confidence, the VRNN-GNN model is closest to an ideal Gaussian. Our proposed combined model is lower in confidence than the VRNN-GNN by $x$\%. We need to investigate this further...} 

\vspace{3pt}

\noindent \textbf{Heuristic Search Policy Analysis: } Next, we investigate how the various filtering approaches perform when the tracking team employs the search heuristic discussed in Section \ref{sec:heuristic}. The heuristic searching policy will help to achieve more detection but will also bring more evasive behaviors of the adversarial agents. We find that the prior-only LL and ADE become worse by 47.07\% and 40.31\% compared with the random policy, and the ADE of Kalman is lower by 45.95\%. This satisfies our motivations to design the two passes. Due to the increase in detection, the performance of the Group I models, such as the GNN, VRNN, VRNN-GNN, and Kalman, are far more comparable with the combined model. The Kalman method is now very close to the combined model (only worse by 3.03\%) compared with the random policy one (worse by 107.6\%), which shows that the combined network will assign a larger weight to the motion model when the detection rate gets high. \Manishawrite{Further, we find that our combined filter model outperforms all our baselines on the confidence threshold metric, despite the individual components being poorer than our baselines. We also note that the confidence of our proposed model has reduced further as compared to the random search heuristic, which is on account of the increase in evasive behavior of the adversary.} 

The overview conclusion we could get is that the running time of the MLP based combined model and simple LSTM model are much smaller than those VRNN or GNN based methods (~$\times$0.1). \Manishawrite{Manisha, We need some comments for the CTP and DESV USING THE TABLES AND THE PLOTS.} 




\begin{figure*}[t]\label{fig:randomBlue}
	\centering
	\includegraphics[scale=0.35]{figs/Filter/filter_metric_random.png}
	\caption{Multiple Filter Evaluations with Random Searching Policy \toedit{reduce y-axis size}}
\end{figure*}

\begin{figure*}[t]\label{fig:heuBlue}
	\centering
	\includegraphics[scale=0.35]{figs/Filter/filter_metric_heu.png}
	\caption{Multiple Filter Evaluations with Heuristic Searching Policy}
\end{figure*}



==> filter_theory.tex <==
\newcommand{\mat}{\boldsymbol}
\section{Filter}\label{sec:filter}

\subsection{Filter System Design}
\toedit{Filtering refers to the estimation of an unobserved state from a past history of observations. In this work, we are interested in developing filtering approaches to predict the state of an adversarial target from past observations of tracking agents.} The reason why the classic filters are not applicable here is due to the loss of information lost from intermittent detections, as we have described in \S\ref{sec:OST}. However, one general framework can be abstracted from those filters: most of them merge different information sources (e.g. prediction and update, multiple motion models, etc.) with some weights (e.g. Kalman gain) for some optimal loss (minimum mean-square error). Following this pattern, we build our filter as two different information branches and a learnable weight to balance them with the negative log-likelihood as the loss function. 

%Most classic linear filters are composed of two main models: prediction and update. The prediction model usually involves a linearized dynamic model and requires the knowledge of control input to generate a dynamically estimated state. A subsequent update model will optimize the predicted state with the current measurement and update state covariance.

The dynamic and observation equations of an agent are usually described as:
\begin{equation}
\mat{x}_k = \mat{F}_k \mat{x}_{k-1} + \mat{B}_k \mat{u}_k + \mat{w}_k
\end{equation}
\begin{equation}
\mat{z}_k = \mat{H}_k \mat{x}_k + \mat{v}_k
\end{equation}
where $\mat{x}_k$ and $\mat{u}_k$ are the state and control input; $\mat{w}_k$ and $\mat{v}_k$ are the process and observation noise, and $\mat{F}_k$, $\mat{B}_k$ and $\mat{H}_k$ is the state transition matrix, control input matrix, and observation matrix at timestep $k$.

In an adversarial environment, however, the opponent's state $\mat{x}_k$ and control input $\mat{u}_k$ \toedit{is only known when the adversary is detected by the \SA{}}. Since we assume accurate detection and a linear forward model, we have
\begin{equation}
\mat{F}_k = \mat{H}_k = \mat{B}_k = \mat{I}, \mat{w}_k = \mat{v}_k = \mat{0}
\end{equation}
and the state (location) of the adversarial agent is estimated as:
\begin{equation}\label{eq:kalman_adv}
\mat{x}_k = \mat{x}_{\hat{k}} + (k - \hat{k})\mat{u}_{\hat{k}}
\end{equation}
where $\hat{k}$ is the latest timestep where detection occurred. This can be shown to satisfy the intermittent Kalman filter estimation \cite{intKalman}.

%Therefore the estimation process has to work in an open loop at timesteps \toedit{when there are no detections}\cite{intKalman}. 
%% We need to propagate the previous state forward when there is no detection update available at the current timestep\cite{intKalman}. 
%Since we assume a linear forward model, the adversarial agent location and velocity can be accurately observed from the detection, we have:
%
%
It seems that equation \eqref{eq:kalman_adv} is the strongest result can be derived in the adversarial settings, however, the adversarial itself may show some patterns and preferences when it achieves its goal. For example, it's goal on reaching certain hideouts, evasive behavior from surveillance, or preference to travel with low terrain cost. This information is also important and can be used as a prior knowledge.

%Compared with linear filters, non-linear filters can deal with non-linear dynamic, non-Gaussian noise and sequence of inputs usually with Maximum a posteriori estimation (MAP) or Maximum likelihood estimation (MLE).

Learning-based filters are more flexible methods compared with their counterparts and are able to consider various temporal and spatial constraints. Many of them are constructed with an encoder-decoder structure from combinations of Recurrent Neural Network (RNN), Variational Auto-Encoders (VAE), Graphical Neural Networks (GNN) and Multi-Layer Perception (MLP) to generate the query variables. In general, it can be presented as:
\begin{eqnarray}
\boldsymbol{e} &=& Encoder(\boldsymbol{z}_{k-T+1:k}) \label{eq:encoder} \\
\boldsymbol{o} &=& Decoder(\boldsymbol{e}) \label{eq:decoder}
\end{eqnarray}
where $\mat{e}$ is the embeddings learned from the input sequence, $\mat{o}$ is the ouput of the neural network and $\mat{z}_{k-T+1:k}$ is the observation sequence from last $T$ timesteps.

Following equation \eqref{eq:encoder}, \eqref{eq:decoder} and the previous analysis, we 
%can input a series of observation to the neural network based filter and expect it to return the state estimation. However, it is not easy to integrate the dynamic prediction (based on occasional detection information) and prior knowledge (based on continuous global environment variables) into one unified network. 
design two separate forward passes called {\textit{prior net}} and {\textit{motion model}} which takes in part of observation and detection, then generates embeddings respectively. We also use another {\textit{confidence net}} to generate weights $\mat{\alpha}$ from the observation to balance the prior and motion embeddings:
\begin{equation}
\mat{G}_e = \mat{\alpha} \mat{p}_h + (\mat{1} - \mat{\alpha}) \mat{m}_h
\end{equation} 
where $\mat{p}_h$, $\mat{m}_h$ and $\mat{G}_e$ are prior, motion and Gaussian embeddings respectively. $\mat{\alpha}$ is the learnable weight.

Since the EA path preferences and bifurcations are encoded in the prior network, the decoder is able to produce multi-hypothesis Gaussians for the state estimation:
\begin{equation}
\mat{\pi}_i, \mat{\mu}_i, \mat{\sigma}_i = Decoder(\mat{e}), i=1, 2, 3, ..., N_g
\end{equation}
where $N_g$ is the number of multiple Gaussian hypothesis and $\pi_i$, $\mu_i$ and $\sigma_i$ are the mixture weight, mean and variance of the mixture component $i$.

\textcolor{red}{Sean's comment: For this section, need a takeaway last paragraph and reference our figure. Also may reorganize such that we present the various components of our filtering model and compare to previous approaches rather than current structure.}



  
\tikzset{global scale/.style={
    scale=#1,
    every node/.append style={scale=#1}
  }
}

\begin{figure}[t]
\centering
\begin{tikzpicture}[global scale = 0.7]
% blocks
\node [draw,
    fill=lightgray,
    minimum width=1cm,
    minimum height=0.6cm,
]  (obs) {Observation};
 
\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm,
    below left=0.5cm and 1.5cm of obs
] (pn) {Prior Net};
 
\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm, 
    below = 0.5cm of obs
]  (cn) {Confidence Net};
 
\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm, 
    below right= 0.5cm and 1.5cm of obs
]  (mn) {Motion Net};

\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm,
    below = 0.5cm of pn
] (ph) {Prior Hidden};
 
\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm, 
    below = 0.5cm of mn
]  (mh) {Motion Hidden};
 
\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm, 
    below = 0.5cm of cn
]  (we) {Weights};

\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm, 
    below = 1.0cm of we
]  (ge) {Gaussian Embedding};

\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm, 
    below = 0.5cm of ge
]  (gp) {Gaussian Parameters ($\pi, \mu, \sigma$)};

% Arrows with text label
\draw[-stealth] (obs.south) to [out=-135,in=90] (pn.north);
\draw[-stealth] (obs.south) -- (cn.north);
\draw[-stealth] (obs.south) to [out=-45,in=90] (mn.north);

\draw[-stealth] (pn.south) -- (ph.north);
\draw[-stealth] (mn.south) -- (mh.north);
\draw[-stealth] (cn.south) -- (we.north);

\draw[-stealth] (we.south) to [out=-160,in=-20] (ph.south);
\draw[-stealth] (we.south) to [out=-20,in=-160] (mh.south);

\draw[-stealth, line width=3pt] ($(we.south)-(0cm, 0.2cm)$) -- ($(ge.north)+(0cm, 0.2cm)$);
\draw[-stealth] (ge.south) -- (gp.north);
\end{tikzpicture}
\caption{Prior-Motion Combined Filter}
\label{fig:posebasedcontrol}
\end{figure}

\begin{comment}
\begin{figure}[t]
\centering
\begin{tikzpicture}[global scale = 0.7]
% blocks
\node [draw,
    fill=lightgray,
    minimum width=1cm,
    minimum height=0.6cm,
]  (bo) {Blue Observation};
 
\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm,
    below=0.5cm of bo
] (mf) {MDN Filter};
 
\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm, 
    below=0.5cm of mf
]  (fo) {$\pi, \mu, \sigma$};
 
\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm, 
    left=0.5cm of fo
]  (bbo) {Base Blue Observation};

\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm,
    below = 1.0cm of bbo
] (policy) {Policy $\pi$};
 
\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm, 
    below = 0.5cm of policy
]  (ba) {Blue Action $a$};
 
\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm, 
    below = 0.5cm of ba
]  (bc) {Blue Critic $Q$};

\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm, 
    below = 1.0cm of bc
]  (pl) {Policy Loss};

\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm, 
    right = 0.5cm of fo
]  (sl) {Supervised Loss};

\node [draw,
    fill=lightgray, 
    minimum width=1cm, 
    minimum height=0.6cm, 
    right = 0.5cm of sl
]  (gtl) {Ground Truth Location};

% Arrows with text label
\draw[-stealth] (bo.south) -- (mf.north);
\draw[-stealth] (mf.south) -- (fo.north);
\draw[-stealth] (fo.south) -- (policy.north);
\draw[-stealth] (policy.south) -- (ba.north);
\draw[-stealth] (ba.south) -- (bc.north);
\draw[-stealth] (bc.south) -- (pl.north);
\draw[-stealth] (fo.east) -- (sl.west);
\draw[-stealth] (gtl.west) -- (sl.east);
\end{tikzpicture}
\caption{Adversarial Search \& Track System Chart}
\label{fig:system}
\end{figure}
\end{comment}

==> marl_exp.tex <==
%\begin{figure}[t]
%\centering
%  %\vspace*{-0.125in}
%  \begin{tikzpicture}[inner sep=0pt, outer sep=0pt]
%  \node[anchor=south west] (RU) at (0in,0in) 
%    {{\includegraphics[width=35pt]{figs/ICRA2021Figs/LongFigs/turn.png}}};
%  \node[anchor=south west,xshift=10pt] (LU) at (RU.south east)
%    {\includegraphics[width=35pt]{figs/ICRA2021Figs/LongFigs/twocircle.png}};
%  \node[anchor=south west,xshift=10pt] (ST) at (LU.south east)
%    {\includegraphics[width=45pt]{figs/ICRA2021Figs/LongFigs/loop.png}};
%  \node[anchor=south west,xshift=10pt] (ZZ) at (ST.south east)
%    {\includegraphics[width=35pt]{figs/ICRA2021Figs/LongFigs/zigzag.png}};
%
%  \node[anchor=north] at (RU.south) {\footnotesize RU};
%  \node[anchor=north] at (LU.south) {\footnotesize LU};
%  \node[anchor=north] at (ST.south) {\footnotesize ST};
%  \node[anchor=north] at (ZZ.south) {\footnotesize ZZ};
%  \end{tikzpicture}
%  \vspace*{-0.5em}
%  \caption{Long-distance trajectories\label{fig:long_trajs}}
%%\end{figure}
%%\begin{figure}[t]
%  \vspace*{0.2em}
%  \centering
%  %\includegraphics[scale=0.13,clip=true,trim=0in 3in 0in 1.25in]{figs/longbox_update.png}
%%  \includegraphics[scale=0.15]{figs/longbox_update.png}
%  {\includegraphics[width=2.5in,clip=true,trim=0in 0in 0in 0in]{figs/Filter/marl_metric.png}}
%  \vspace*{-0.5em}
%  \caption{MADDPG benchmarking results\label{fig:longbench}}
%  \vspace*{-1em}
%\end{figure}

\subsection{Experiments and Results\label{sec:longDist_exp}}

\todo{Talk about how our combined filtering model outperforms all other baselines and deals with the changing data distribution that occurs during training.}

\todo{include table of average results}

\begin{figure*}[t]\label{fig:marl_metrics}
	\centering
	\includegraphics[scale=0.35]{figs/Filter/marl_metric.png}
	\caption{MARL + Filtering results: We show our combined filtering model + MADDPG outperforms all other baselines. \toedit{including one more baseline + renaming legend}}
\end{figure*}


\subsubsection{Results and Analysis}





==> marl_theory.tex <==
\begin{figure*}[t]
  \vspace*{0.2em}
  \centering
  {\includegraphics[width=1.2in,clip=true,trim=0in 0in 0in 0in]{figs/Filter/Interception_meet.png}}
  {\includegraphics[width=1.2in,clip=true,trim=0in 0in 0in 0in]{figs/Filter/Interception_catch.png}}
  {\includegraphics[width=1.2in,clip=true,trim=0in 0in 0in 0in]{figs/Filter/spiral.png}}
  {\includegraphics[width=1.2in,clip=true,trim=0in 0in 0in 0in]{figs/Filter/one_step.png}}
  {\includegraphics[width=1.2in,clip=true,trim=0in 0in 0in 0in]{figs/Filter/random.png}}
  \vspace*{-0.5em}
  \caption{Heuristic Plots (\todo{under revison})\label{fig:longbench}}
  \vspace*{-1em}
\end{figure*}
\section{MADDPG Informed by MDN Filter}\label{sec:MADDPG}
In this section, we will discuss the strategies we are using in the \ST{} task and how the new designed PMC filter is used to help on its efficiency and accuracy. Generally speaking, we are using three groups of strategies here: MDN informed MARL, MARL without MDN, and heuristics. Ablation experiments are used to show the MARL with the PMC filter can outperform other methods with respect to the detection rate, closest distance and rewards.
\subsection{Motivation}
\toedit{Even though we already build heuristic policies considering the previous works}


\subsection{Multi-agent Reinforcement Learning}
Multi-agent deep deterministic policy gradient (MADDPG) is a multi-agent extension of the basic Deep Deterministic Policy Gradient (DDPG) reinforcement learning algorithm and follows the off-policy centralized training and decentralized execution paradigm. Each agent has its own actor-critic structure but the critic could take the combination of the state-action of all agents compared with the input of the actor which is each own experience tuple. 
 
We use MADDPG as our framework to train the agent policies. The base \SA observation includes the current timestep, its own current location, current locations of all other \SA and the location of known hideouts. We call the base observatio $O_b$. The second part of the observation is named augmenting part $O_a$ which may include the last two detections with velocities or the Gaussians from the filter in the searching agent local frame:
\begin{equation}
\mu^{loc}_{j} = \mu_j - x_s, j=1,2,3,...,N_g
\end{equation} 
where $N_g$ is the number of multiple Gaussians.
Then we can present the augmented observation of agent $i$ as $O_i = [O_b \Vert O_a]$. Then the action of the agent $i$ could be calculated using its own policy:
\begin{equation}
a_i = \pi_i(O_i), i=1,2,...,N_a
\end{equation}
where $N_a$ is the number of search agents.
Then the critic could be updated with TD error between two consecutive timesteps. The loss function $L(\theta_{i})$ is written as:
 \begin{equation}
 \begin{split}
 L(\theta_{i})=\mathbb{E}_{x,a,r,x^{\prime}}[(Q_{i}^{\pi}(x,a_{1},...,a_{N})-y)^{2}]
 \end{split}
 \end{equation}
 \begin{equation}
 \begin{split}
 y=r_{i}+\gamma Q_{i}^{\pi^{\prime}}(x^{\prime},a_{1}^{\prime},...,a_{N}^{\prime})\vert \pi^{\prime}(a_{i}\vert o_{i})
 \end{split}
 \end{equation}
Then the policy could be updated with the gradient:

 \begin{multline}
 \nabla_{\theta_{i}}J(\mu_{i})
 =\mathbb{E}_{x,a\sim \mathcal{D}}[\nabla_{\mu_{i}}\pi_{i}(a_{i}\vert o_{i}) \\ 
 \nabla_{a_{i}}Q_{i}^{\pi}(x,a_{1},...,a_{N})\vert \pi_{i}(a_{i}\vert o_{i})]
 \end{multline}

 where $\gamma$ is discount factor. $\theta_{i},\mu_{i}, i=1,2,...,N$ are the parameters of the neural network critic and actor $Q_{i}, \pi_{i}$ respectively. $x$ is the combination of all agents' observation $x=(o_{1},o_{2},...,o_{N})$. Since we are using deterministic policy, $a_{i}=\pi_{i}(a_{i}\vert o_{i})=\pi_{i}(o_{i})$ is an action vector instead of a distribution. Since the ground truth state distribution is not accessible, we need to save to and draw samples from the replay buffer $\mathcal{D}$. Superscript prime means the quantity is of the next timestep. Subscript indicates the agent index and it means 'for all agents' if there is no such index.
\newcommand{\trajTimeStart}[1]{t_{#1,s}}
\newcommand{\trajTimeEnd}[1]{t_{#1,e}}
\newcommand{\featureTraj}[1]{\featureSetD_{#1} (t) |_{\trajTimeStart{#1}}^{\trajTimeEnd{#1}}}

%\begin{table*}[t]
%  \vspace*{0.06in}
%  \centering
%  \addtolength{\tabcolsep}{-3pt}
%  \begin{minipage}[t]{0.24\textwidth}
%  \centering
%  \caption{\textrm{Tracking ATE (cm)}\label{tb:longTrajBench}}
%  \begin{tabular}{|c||ccc|}
%    \hline 
%    \textbf{Seq.} & PO & SLAM & TS \\ 
%    \hline 
%%      & \textcolor{white}{$v,\omega$} & & \\
%    RU & 2.40  & 6.19   & 4.02  \\ 
%    LU & 3.47  & 17.22  & 7.30  \\ 
%    ST & 2.25  & 7.95   & 6.06  \\ 
%    ZZ & 5.19  & 11.01  & 8.30  \\ 
%    \hline 
%    \textbf{Avg. ATE} & \textbf{3.33} & 10.59 & {\em 6.42} \\ 
%    \hline 
%  \end{tabular}
%  \end{minipage}
%  \begin{minipage}[t]{0.2\textwidth}
%    \centering
%    \caption{\textrm{Terminal Error (cm)}%
%    \label{tb:longTrajTE}}
%    \begin{tabular}{|c||ccc|}
%    \hline 
%    \textbf{Seq.} & PO & SLAM & TS \\ 
%    \hline 
%%      & \textcolor{white}{$v,\omega$} & & \\
%    RU & 2.33  & 11.61  & 6.77  \\ 
%    LU & 3.14  & 26.06  & 18.90  \\ 
%    ST & 2.38  & 8.61   & 7.74  \\ 
%    ZZ & 4.28  & 5.22   & 7.18  \\ 
%    \hline 
%    \textbf{Avg.} & \textbf{3.03} & 12.88 & \em 10.15 \\ 
%    %\textbf{Std. ATE} & 0.0000 & 0.0000 & 0.0000 \\
%    \hline 
%    \end{tabular}
%  \end{minipage}
%  \begin{minipage}[t]{0.18\textwidth}
%  \centering
%  \caption{\textrm{Estimation ATE (cm)}%
%  \label{tb:longEst}}
%  \begin{tabular}{|c||cc|}
%    \hline 
%    \textbf{Seq.} & SLAM & TS \\ 
%    \hline 
%%     & \textcolor{white}{$v,\omega$} & \\
%    RU & 9.15  & 8.49 \\ 
%    LU & 13.68 & 11.09 \\ 
%    ST & 7.00  & 7.96 \\ 
%    ZZ & 12.13 & 10.37 \\ 
%    \hline 
%    \textbf{Avg.} & 10.49 & \textbf{\em 9.48}\\ 
%    \hline 
%  \end{tabular}
%  \end{minipage}
%  \begin{minipage}[t]{0.35\textwidth}
%  \centering
%  \caption{\textrm{Control Effort} \label{tb:longCost}}
%  \begin{tabular}{|c||cccccc|}
%    \hline 
%    \textbf{Seq.} & \multicolumn{2}{c}{PO} & \multicolumn{2}{c}{SLAM} & \multicolumn{2}{c|}{TS}\\ 
%    \hline 
%    • & $\nu$ & $\omega$ & $\nu$ & $\omega$ & $\nu$ & $\omega$\\ 
%    RU & 15.51 & 14.95 & 13.94 & 12.08 & 11.94 & 10.80 \\ 
%    LU & 17.77 & 9.53  & 16.38 & 9.24  & 13.67 & 9.94 \\ 
%    ST & 17.80 & 13.87 & 16.00 & 12.96 & 13.74 & 12.29 \\ 
%    ZZ & 23.17 & 11.73 & 21.00 & 10.67 & 17.97 & 10.89 \\ 
%    \hline 
%    \textbf{Avg.} & 18.56 & 12.52 & 16.83 & 11.24 & \textbf{\em 14.33} & \textbf{\textit{10.98}}\\
%    • & \multicolumn{2}{c}{31.08} & \multicolumn{2}{c}{28.07} & \multicolumn{2}{c|}{\textbf{\em 25.31}} \\
%  \hline 
%  \end{tabular} 
%  \end{minipage}
%  \addtolength{\tabcolsep}{2pt}
%  \vspace*{-0.15in}
%\end{table*}

% \begin{figure}[t]
% \centering
%   \vspace*{0.15in}
%   \begin{tikzpicture}[inner sep=0pt, outer sep=0pt]
%   \node[anchor=south west] (orig) at (0in,0in) 
%     {{\includegraphics[width=0.8\columnwidth]{figs/feature_replenishment.png}}};
  
%   % landmarks
%   \node[anchor=west] (ti2_f) at ($(orig.west) + (-0.2in, 0.3in)$) {\footnotesize $\pointSet^{\mc W}(\trajTimeEnd{i-2})$};
%   \node[anchor=west] (ti1_f) at ($(orig.west) + (0.7in, 0.3in)$) {\footnotesize $\pointSet^{\mc W}(\trajTimeEnd{i-1})$};
%   \node[anchor=west] (ti_f) at ($(orig.west) + (1.4in, 0.3in)$) {\footnotesize $\pointSet^{\mc W}(\trajTimeEnd{i})$};
  
%   % time
%   \node[anchor=north] (ti21) at ($(ti2_f.south) + (0.05in, -0.4in)$) {\footnotesize $\trajTimeEnd{i-2}$};
%   \node[anchor=north] (ti22) at ($(ti21.south) + (0in, 0in)$) {\footnotesize $\trajTimeStart{i-1}$};
%   \node[anchor=north] (ti11) at ($(ti1_f.south) + (0.05in, -0.4in)$) {\footnotesize $\trajTimeEnd{i-1}$};
%   \node[anchor=north] (ti12) at ($(ti11.south) + (0in, 0in)$) {\footnotesize $\trajTimeStart{i}$};
%   \node[anchor=north] (ti1) at ($(ti_f.south) + (0in, -0.4in)$) {\footnotesize $\trajTimeEnd{i}$};
%   \node[anchor=north] (ti2) at ($(ti1.south) + (0in, 0in)$) {\footnotesize $\trajTimeStart{i+1}$};
  
%   % feature traj
%   \node[anchor=north] (tib_ft) at ($(orig.west) + (0.6in, -0.45in)$) {\footnotesize $\featureTraj{i-1}$};
%   \node[anchor=north] (ti_ft) at ($(orig.west) + (1.3in, -0.45in)$) {\footnotesize $\featureTraj{i}$};
%   \node[anchor=north] (tin_ft) at ($(orig.west) + (2.1in, -0.45in)$) {\footnotesize $\featureTraj{i+1}$};
  
%   % arrows
% %  \draw[->, dashed] (ti21.north) -- ($(ti21.north) + (0in, 0.1in)$);
% %  \draw[->, dashed] (ti11.north) -- ($(ti11.north) + (0in, 0.08in)$);
% %  \draw[->, dashed] (ti1.north) -- ($(ti1.north) + (0in, 0.2in)$);
  
%   \draw[->, very thick] (tib_ft.north) -- ($(tib_ft.north) + (0in, 0.2in)$);
%   \draw[->, very thick] (ti_ft.north) -- ($(ti_ft.north) + (0in, 0.5in)$);
%   \draw[->, very thick] (tin_ft.north) -- ($(tin_ft.north) + (0in, 0.2in)$);
	
%   \end{tikzpicture}
%   \caption{Feature replenishment process. There are three segments of feature trajectories. Stars are observed point sets at corresponding time. Each circle is the start or end time of next or this segment of feature trajectory. Three feature trajectories are generated by the feature replenishment equation \eqref{eq:trajReg}. \label{fig:feat_rep}}
%   \vspace*{-1em}
% \end{figure}

\tikzset{global scale/.style={
    scale=#1,
    every node/.append style={scale=#1}
  }
}

% \begin {figure}
% \vspace*{-1em}
% \centering
% %\begin{adjustbox}{width=\textwidth}
% \begin{tikzpicture}[global scale = 0.7]
% % Sum shape
% \node [draw,
%     fill=Goldenrod,
%     minimum width=1.5cm,
%     minimum height=1cm,
%     text width=2.5cm,
%     text centered
% ]  (FG) at (0,0) {\centering Feature \\ Replenishment};

% \node[draw,
%     circle,
%     minimum size=0.6cm,
%     fill=Rhodamine!50,
%     right=0.5cm of FG
% ] (sum){};
 
% \draw (sum.north east) -- (sum.south west)
%     (sum.north west) -- (sum.south east);
 
% \draw (sum.north east) -- (sum.south west)
% (sum.north west) -- (sum.south east);
 
% \node[left=-1pt] at (sum.center){\tiny $+$};
% \node[below] at (sum.center){\tiny $-$};
 
% % Controller
% \node [draw,
%     fill=Goldenrod,
%     minimum width=1.5cm,
%     minimum height=1cm,
%     text width=2cm,
%     text centered,
%     right=0.5cm of sum
% ]  (controller) {\centering Trajectory \\ Servoing};
 
% % System H(s)
% \node [draw,
%     fill=SpringGreen, 
%     minimum width=1.5cm,
%     minimum height=1cm,
%     right=0.7cm of controller
% ] (system) {Plant};
 
% % Sensor block
% \node [draw,
%     fill=SeaGreen, 
%     minimum width=1.5cm,
%     minimum height=1cm,
%     below right= 0.4cm and -0.8cm of controller
% ]  (sensor) {Tracked Features};

% \node [draw,
%     fill=SeaGreen, 
%     minimum width=1.5cm,
%     minimum height=1cm,
%     below right= 1.5cm and -1.1cm of controller
% ]  (SLAM) {V-SLAM Pose};
 
% % Arrows with text label
% \draw[-stealth] (sum.east) -- (controller.west)
%     node[midway,above]{$e$};
 
% \draw[-stealth] (controller.east) -- (system.west) 
%     node[midway,above]{$\dot{\featSetV},u$};
    
% \draw[-stealth] ($(controller.north) + (0in, 0.3in)$) -- (controller.north)
%     node[midway,right]{$u^*$};
 
% \draw[-stealth] (system.east) -- ++ (1.25,0) 
%     node[midway](output){}node[midway,above]{$\featSetV,\mcframe{\roboF}{W}{R}$};
 
% \draw[-stealth] (output.center) |- (sensor.east);
 
% \draw[-stealth] (sensor.west) -| (sum.south) 
%     node[near end,left]{$\hat{\featSetV}$};
 
% \draw [-stealth](FG) --(sum.west) 
%     node[midway,above]{$\featSetDV$};
    
% \draw [-stealth] ($(FG.west) + (-1.5,0)$) -- (FG.west)
%     node[midway,above]{Ref Traj};
    
     
% \draw[-stealth] (output.center) |- (SLAM.east);
 
% \draw[-stealth] (SLAM.west) -| (FG.south) 
%     node[near end,left]{$\hat{{\roboF}}^{\mc{W}}_{\mc{R}}$};
% \end{tikzpicture}
% \caption{Block Diagram for long-term Trajectory Servoing \label{fig:BlockTS}}

% %\end{adjustbox}
% \end{figure}


